One Net Fits All: A unifying semantics of Dynamic Fault Trees using GSPNs

Dynamic Fault Trees (DFTs) are a prominent model in reliability engineering. They are strictly more expressive than static fault trees, but this comes at a price: their interpretation is non-trivial and leaves quite some freedom. This paper presents a GSPN semantics for DFTs. This semantics is rather simple and compositional. The key feature is that this GSPN semantics unifies all existing DFT semantics from the literature. All semantic variants can be obtained by choosing appropriate priorities and treatment of non-determinism.

==> Makefile <==
# Copyright 2004 Chris Monson (shiblon@gmail.com)
# Latest version available at http://www.bouncingchairs.net/oss
#
#    This file is part of ``Chris Monson's Free Software''.
#
#    ``Chris Monson's Free Software'' is free software; you can redistribute it
#    and/or modify it under the terms of the GNU General Public License as
#    published by the Free Software Foundation, Version 2.
#
#    ``Chris Monson's Free Software'' is distributed in the hope that it will
#    be useful, but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
#    Public License for more details.
#
#    You should have received a copy of the GNU General Public License along
#    with ``Chris Monson's Free Software''; if not, write to the Free Software
#    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA
#
#    It is also available on the web at http://www.gnu.org/copyleft/gpl.html
#
#    Note that using this makefile to build your documents does NOT place them
#    under the GPL unless you, the author, specifically do so.  In other words,
#    I, Chris Monson, the copyright holder and author of this makefile,
#    consider it impossible to ``link'' to this makefile in any way covered by
#    the GPL.
#
#
# TO OBTAIN INSTRUCTIONS FOR USING THIS FILE, RUN:
#    make help
#
fileinfo	:= LaTeX Makefile
author		:= Chris Monson
version		:= 2.2.0
#
.DEFAULT_GOAL	:= all
# Note that the user-global version is imported *after* the source directory,
# so that you can use stuff like ?= to get proper override behavior.
.PHONY: Makefile GNUmakefile Makefile.ini $(HOME)/.latex-makefile/Makefile.ini
-include Makefile.ini
-include $(HOME)/.latex-makefile/Makefile.ini
# Better names for these things
.PHONY: Variables.ini $(HOME)/.latex-makefile/Variables.ini
-include Variables.ini
-include $(HOME)/.latex-makefile/Variables.ini
#
# This can be pdflatex or latex - you can change this by adding the following line to your Makefile.ini:
# BUILD_STRATEGY := latex
BUILD_STRATEGY		?= pdflatex
#
# Sets LC_ALL=C, by default, so that the locale-aware tools, like sort, be
# # immune to changes to the locale in the user environment.
export LC_ALL		?= C
#
#
# If you specify sources here, all other files with the same suffix
# will be treated as if they were _include_ files.
onlysources.tex	?= main.tex
#onlysources.tex.sh	?=
#onlysources.tex.pl	?=
#onlysources.tex.py	?=
#onlysources.rst	?=
#onlysources.fig	?=
#onlysources.gpi	?=
#onlysources.dot	?=
#onlysources.xvg	?=
#onlysources.svg	?=
#onlysources.eps.gz	?=
#onlysources.eps	?=
#
# If you list files here, they will be treated as _include_ files
#includes.tex		?= file1.tex file2.tex
#includes.tex.sh	?=
#includes.tex.pl	?=
#includes.tex.py	?=
#includes.rst		?=
#includes.fig		?=
#includes.gpi		?=
#includes.dot		?=
#includes.xvg		?=
#includes.svg		?=
#includes.eps.gz	?=
#includes.eps		?=
#
# If you list files or wildcards here, they will *not* be cleaned - default is
# to allow everything to be cleaned.
#neverclean		?= *.pdf
#
# Alternatively (recommended), you can add those lines to a Makefile.ini file
# and it will get picked up automatically without your having to edit this
# Makefile.
#
# KNOWN ISSUES:
# * The following occurs:
#   file with: \usepackage{named}\bibliographystyle{named}
#   Compile
#   change to: \usepackage{apalike}\bibliographystyle{apalike}
#   Compile again -- BARF!
#
#   The workaround: make clean-nographics; make
#
#   Note that we may not be able to fix this.  LaTeX itself barfs
#   on this, not the makefile.  The very first invocation of LaTeX
#   (when something like this has happened) reads the existing .aux
#   file and discovers invalid commands like \citeauthoryear that
#   are only valid in the package that was just removed.  It then
#   tries to parse them and explodes.  It's not at all clear to me
#   how to fix this.  I tried removing the .aux files on the first
#   run of LaTeX, but that necessarily requires more subsequent
#   rebuilds on common edits.  There does not appear to be a
#   graceful solution to this issue.
#
#
# CHANGES:
# Chris Monson (2011-05-20):
# * Bumped version to 2.2.0 (release!)
# Chris Monson (2011-05-19):
# * Bumped version to 2.2.0-rc15
# * Issue 125: infinite recursion with nomenclature files
# * Issue 125: removed .d as a target for .nls in get-log-index
# * Cleaned up invocation of run-makeindex to take an optional .ist instead of flags.
# Chris Monson (2011-04-06):
# * Bumped version to 2.2.0-rc14
# * Issue 121: Added Targets.ini and corresponding help text for it.
# * Issue 121: Added Variables.ini (Makefile.ini still works, though).
# * Issue 121: Added .DEFAULT_GOAL optional setting.
# * Issue 120: xindy compatibility
# Chris Monson (2011-03-16):
# * Bumped version to 2.2.0-rc13
# * Fixed a bug in kspewhich invocation - random characters and a missing pipe.
# * Added font embedding to gnuplot output.
# Chris Monson (2011-03-15):
# * Bumped version to 2.2.0-rc12
# * Issue 119: Annoying warning from which if Gnuplot not installed.
# * Fixed catchall error output to show more info from the log.  Cutting off the
#     first line is too jarring.
# * Issue 118: Better glossary support
# Chris Monson (2011-03-03):
# * Bumped version to 2.2.0-rc11
# * Issue 112: Fixed regression introduced by use of cygpath (ugly warnings)
# Chris Monson (2011-02-03):
# * Bumped version to 2.2.0-rc10
# * Issue 112: Added path normalization for cygwin systems
# * Fixed a bug in get-missing-inputs where we weren't specifying target files
# Chris Monson (2011-01-24):
# * Issue 111: Added .jpeg as a possible image extension
# Chris Monson (2011-01-21):
# * Issue 110: Long filenames not produced correctly in .d file
# * Fixed problem with unknown control sequence error parsing
# * Fixed problem with \r in fatal output (was interpreted as LF by echo)
# * Removed a spurious "hi"
# Chris Monson (2011-01-14):
# * Bumped version to 2.2.0-rc8
# * Issue 107: Removed comment with embedded newline, fixing MinGW on Windows 7.
# Chris Monson (2011-01-07):
# * Emit an error if .gpi.d files have dependencies with : in the name
# Chris Monson (2011-01-05):
# * Bumped version to 2.2.0-rc7
# * Issue 106: existing graphic dependencies not generated correctly
# Chris Monson (2011-01-04):
# * Issue 106: not cleaning eps log files properly
# * Issue 106: not rebuilding after creating .pdf graphics from .eps
# * Issue 94: svg going unnecessarily through eps (can't reproduce)
# Chris Monson (2010-12-31):
# * Issue 100: make hanging because of faulty graphics detection (sed bug)
# * Issue 108: do not ignore fatal errors from pdftex
# Chris Monson (2010-12-23):
# * Added gpi_global to gnuplot dependencies so that changes are detected
# Chris Monson (2010-12-20):
# * Updated build file to be smarter about Python version detection
# * Created a bunch of test files and supporting scripts
# * Issue 72: added apacite capaability (thanks to matkarat)
# Chris Monson (2010-11-23):
# * Changed to multi-part makefile build (split out sed scripts)
# * Added build script and supporting infrastructure
# * Updated test directory format
# * Added notes about needed test cases
# * Changed to use -file-line-error and fixed multiple inclusion/error bugs
# * Added run_sed.py to allow easy testing of sed scripts outside of make
# Chris Monson (2010-11-11):
# * Bumped version to 2.2.0-rc7
# * issue 92: broken hyperref driver detection fixed
# * issue 101: Broken inkscape conversion
# * issue 102: Broken specification of font size for gnuplot pdfcairo
# * Added KEEP_TEMP so that we can avoid deleting useful temporaries for debugging
# * Restructured gnuplot code to be easier to follow
# * Fixed a bug in convert-gpi where we were using $< instead of $1
# Chris Monson (2010-11-03):
# * Bumped version to 2.2.0-rc6
# * issue 96: Fix sed errors when using make variables in substitutions
# Chris Monson (2010-07-28):
# * Bumped version to 2.2.0-rc5 (rc4 is broken)
# * Bail out when we find the use of the import.sty package
# * Issue 90: Add -z to dvips invocation
# * Issue 67: Add xelatex support (thanks to Nikolai Prokoschenko for the patch!)
# * Issue 85: Add warning about make 3.80
# Chris Monson (2010-06-20):
# * Bumped version to 2.2.0-rc3
# * Attempt to fix bug with ! error detection (issue 88)
# * Added svg->pdf direct support (issue 89)
# Chris Monson (2010-04-28):
# * Bumped version to 2.2.0-rc2
# * Fixed %._show target
# Chris Monson (2010-04-08):
# * Bumped version to 2.2.0-rc1
# * Added back in the rst_style_file stuff that got broken when switching
#     rst -> tex to use the script mechanism
# Chris Monson (2010-03-23):
# * Bumped version to 2.2.0-beta8
# * Work on issue 76: bad backtick escape for some sed versions, failure
#     to clear out the hold buffer when outputting MISSING comment.
#     - Backed out 2>&1 to &> (doesn't work in sh)
#     - Backed out using . to source variables
# Chris Monson (2010-03-22):
# * Bumped version to 2.2.0-beta7
# * Issue 72: Fix latex/bibtex invocation order for annotated bib styles
# * Fixed informational output to reflect which LaTeX run we're on
# * Fixed graphic detection to include graphics that are already there in
#     .d files
# * Tightened up the .d file output to only make .d depend on graphic
#     *source* files.  This means that building foo.d no longer
#     builds all of the graphics files on which foo.tex depends.
#     Had to use .SECONDEXPANSION trickery to make it work.
# * Changed get-graphics to only accept a stem.
# * Fixed build-once logic for scripted .tex to work better
# * Made get-inputs sed script more maintainable.
# * Moved Makefile.ini import up higher.
# * Changed bare stems to not recursively invoke make
# * Updated diff output to be more silent everywhere
# * Added a MISSING comment to the .d file if stuff isn't found - forces
#     removal of .1st.make file, which often forces it to try again.
# * Fixed broken graphics-target function
# * Added sleep to .d file generation when stuff is missing - if it
#     builds too fast, make doesn't realize it needs to be reloaded,
#     and thus never discovers some deeper dependencies (especially
#     evident when graphics are included from scripted include
#     files).
# Chris Monson (2010-03-17):
# * Bumped version to 2.2.0-beta6
# * Fixed bareword builds to actually work (requires static patterns)
# * Fixed colorization to work with new paragraph stuff
# Chris Monson (2010-03-17):
# * Bumped version to 2.2.0-beta5
# * Fixed graphic detection to be much more focused - splits log file
#     into paragraphs before doing pattern matching.
# * Fixed make foo to work properly (recursively calls make foo.pdf)
# * Fixed gpi -> pdf generation to not waste time building .eps *after*
#     the pdf already exists.
# * Changed log copies to include MAKE_RESTARTS as part of the name.
# * Fixed missing include file detection (also makes use of the paragraph
#     stuff) to detect missing scripted include files.
# Chris Monson (2010-03-16):
# * Bumped version to 2.2.0-beta4
# * issue 70: .pdf not moved out of the way properly on first
#     compilation, resulting in early error detection failure.
# * issue 74: fixed broken error on missing .aux files: the
#     implementation was masking real errors.
# Chris Monson (2010-03-15):
# * Bumped version to 2.2.0-beta3
# * issue 71: Made the tput dependency optional
# * issue 73: Made .tex targets not pull in .d files (building them from
#     scripts should not require a .d)
# * issue 74: Output a much saner error when a .aux file is not produced
#     (e.g., when you are typing "make" without arguments in a
#     directory with included .tex files that are not named with
#     ._include_.)
# Chris Monson (2010-03-11):
# * Bumped version to 2.2.0-beta2
# * Fixed clean-graphics to get rid of intermediate .eps files that may
#     be hanging around
# * Added an automatic setting to use eps terminals in pdflatex mode for
#     gnuplot if it doesn't understand pdf.
# * issue 66: Removed grayscale generation via magic suffix.  Grayscale
#     generation is now only available via GRAY=1
# * issue 68: Added explicit handling of LC_ALL for locale-aware tools
#     like "sort"
# Chris Monson (2010-03-10):
# * Bumped version to 2.2.0-beta1
# * Fixed success message to handle output message in different places
# * Added name of produced file to success message
# Chris Monson (2010-03-10):
# * Bumped version to 2.2.0-alpha3
# * Added meaningful error message for wrong hyperref options
# * Added meaningful error message for incorrect graphics extensions
# Chris Monson (2010-03-09):
# * Bumped version to 2.2.0-alpha2
# * Updated graphics handling (gnuplot and fig generate pdf natively)
# * Changed xmgrace to output monochrome natively
# Chris Monson (2010-03-09):
# * Bumped version to 2.2.0-alpha1 - major change!
# * Support pdflatex natively and by default (issue 6 - a long time coming)
# * Add ability to have a single $HOME/.latex-makefile/Makefile.ini for
#     all invocations
# * Reworked graphic inclusion detection so that extensions need not be
#     specified for either build strategy (e.g.,
#     \includegraphics{test1.eps} -> \includegrahpics{test1})
# * Changed log format to include filenames and line numbers
# Chris Monson (2010-02-04):
# * Bumped version to 2.1.43
# * All of the following are for issue 63 (thanks to mojoh81):
# * Added documentation about fixing Makefile.ini default target
# * Added perl and python script targets
# * Fixed run logic to allow included .tex files to be scripted (the
#     run-again logic now detects missing .tex files, and the MV
#     command has been switched out for a command that only invokes
#     MV if the files exist)
# * Changed scripted generation to only run once per make invocation
# * Added dependency on expr
# Chris Monson (2010-01-19):
# * Bumped version to 2.1.42
# * issue 62: Added .brf extension to cleanable files (backrefs)
# Chris Monson (2010-01-07):
# * Bumped version to 2.1.41
# * issue 60: bad makeindex runs now error out on subsequent tries
# Chris Monson (2009-12-01):
# * Bumped version to 2.1.40
# * issue 36: build all indices (for e.g., splitidx usage)
# * issue 59: clean up all generated files (including indices)
# Chris Monson (2009-11-23):
# * Bumped version to 2.1.39
# * issue 57: change ps2pdf invocations to just use gs directly
# Chris Monson (2009-11-19):
# * Bumped version to 2.1.38
# * issue 57: Added some limited support for Cygwin (spaces in filenames)
# Chris Monson (2009-11-15):
# * Bumped version to 2.1.37
# * Removed svninfo, since this is now managed by mercurial
# * Fixed typo in changelist
# * Issue 52: added jpg->eps conversion (thanks to brubakee)
# * Issue 54: fix missing Overfull colorization due to lack of a blank
#     line preceding the first error.
# * Issue 51: remove head.tmp and body.tmp in make clean invocation
# * Issue 56: maintain multiple versions of log files (for debugging)
# Chris Monson (2009-11-14):
# * Bumped version to 2.1.36
# * Issues 53 and 49: added .brf, .mtc, and .maf to the cleanables
# Chris Monson (2009-11-05):
# * Bumped version to 2.1.35
# * Added nomenclature support (see issue 48)
# Chris Monson (2009-10-29):
# * Bumped version to 2.1.34
# * Fixed _out_ creation bug introduced in 2.1.33 (it was always created)
# * Fixed erroneous help output for $HOME in BINARY_TARGET_DIR
# * Changed contact email address - bring on the spam!
# Chris Monson (2009-10-21):
# * Bumped version to 2.1.33
# * Fixed issue 46, adding support for dot2tex (thanks to fdemesmay)
# * Made all_files.* settable in Makefile.ini (using ?= instead of :=)
# * Fixed issue 47, thanks to fdemesmay: add binary copy directory, copy
#     dvi, pdf, and ps if it exists
# Chris Monson (2009-09-25):
# * Bumped version to 2.1.32
# * Fixed so that a changed lol file will cause a rebuild
# * Added .lol files to the cleanable list
# Chris Monson (2009-09-08):
# * Bumped version to 2.1.31
# * Closed issue 43: evince doesn't notice pdf change w/out touch
# Chris Monson (2009-08-28):
# * Bumped version to 2.1.30
# * Closed issue 39: Capture multi-line log warnings/errors to output
# Chris Monson (2009-08-26):
# * Bumped version to 2.1.29
# * Closed issue 42: add svg support using inkscape
# Chris Monson (2009-08-17):
# * Bumped version to 2.1.28
# * Patch from paul.biggar for issue 38: package warnings are overlooked
# Chris Monson (2009-08-07):
# * Bumped version to 2.1.27
# * Included patch for issue 37 - removes pdf/ps files before copying,
#     allowing some broken viewers to see changes properly.
# Chris Monson (2009-05-15):
# * Bumped version to 2.1.26
# * Included patch for issue 9 from favonia - detects .fig changes for
#     pstex files during regular compilation, so long as the pstex
#     has been built at least once with make all-pstex.
# Chris Monson (2009-03-27):
# * Bumped version to 2.1.25
# * Cleaned up a bunch of variable setting stuff - more stuff is now
#     settable from Makefile.ini
# * Cleaned up documentation for various features, especially settable
#     variables.
# * issue 28: support for png -> eps conversion (it even looks good!)
# * issue 29: support for "neverclean" files in Makefile.ini
# * issue 30: make ps2pdf14 the default - fall back when not there
# Chris Monson (2009-03-09):
# * Bumped version to 2.1.24
# * issue 27: xmgrace support (thanks to rolandschulzhd)
# Chris Monson (2008-10-23):
# * Bumped version to 2.1.23
# * issue 23: fixed _check_programs to not use bash string subs
# Chris Monson (2008-09-02):
# * Bumped version to 2.1.22
# * Appled patch from Holger <yllohy@googlemail.com> to add include
#     sources and some documentation updates.
# * Updated backup_patterns to be a bit more aggressive (also thanks to
#     Holger)
# Chris Monson (2008-08-30):
# * Bumped version to 2.1.21
# * Added ability to specify onlysources.* variables to indicate the only
#     files that should *not* be considered includes.  Thanks to Holger
#     <yllohy@googlemail.com> for this patch.
# * Added an automatic include of Makefile.ini if it exists.  Allows
#     settings to be made outside of this makefile.
# Chris Monson (2008-05-21):
# * Bumped version to 2.1.20
# * Added manual pstex compilation support (run make all-pstex first)
# * Removed all automatic pstex support.  It was totally breaking
#     everything and is very hard to incorporate into the makefile
#     concept because it requires LaTeX to *fail* before it can
#     determine that it needs the files.
# Chris Monson (2008-04-17):
# * Bumped version to 2.1.19
# * Changed the pstex build hack to be on by default
# Chris Monson (2008-04-09):
# * Bumped version to 2.1.18
# * issue 16: fixed pstex build problems, seems nondeterministic.  Added
#     gratuitious hack for testing: set PSTEX_BUILD_ALL_HACK=1.
# Chris Monson (2008-04-09):
# * Bumped version to 2.1.17
# * issue 20: fixed accumulation of <pid>*.make files - wildcard was
#     refusing to work on files that are very recently created.
# Chris Monson (2008-04-02):
# * Bumped version to 2.1.16
# * issue 19: Removed the use of "type" to fix broken "echo" settings
# Chris Monson (2008-03-27):
# * Bumped version to 2.1.15
# * issue 18: Favors binary echo over builtin, as binary understands -n
# * issue 16: Fixed handling of missing pstex_t files in the log
# * issue 9: Added .SECONDARY target for .pstex files
# Chris Monson (2008-03-21):
# * Bumped version to 2.1.14
# * Fixed broken aux file flattening, which caused included bibs to be
#     missed.
# Chris Monson (2008-03-20):
# * Bumped version to 2.1.13
# * Changed error output colorization to show errors for missing files
#     that are not graphics files.
# Chris Monson (2008-03-20):
# * Bumped version to 2.1.12
# * Fixed a regression introduced in r28 that makes bibtex fail when
#     there is no index file present
# Chris Monson (2008-03-03):
# * Bumped version to 2.1.11
# * Fixed issue 11 (handle index files, reported by abachn)
# * Cleaned up some comments and help text
# Chris Monson (2008-01-24):
# * Bumped version to 2.1.10
# * Fixed to work when 'sh' is a POSIX shell like 'dash'
# Chris Monson (2007-12-12):
# * Bumped version to 2.1.9
# * Fixed documentation and dependency graph for pstex files
# Chris Monson (2007-12-12):
# * Bumped version to 2.1.8
# * Added basic pstex_t support for fig files (Issue 9 by favonia)
#     I still suggest that psfrag be used instead.
# Chris Monson (2007-10-16):
# * Bumped version to 2.1.7
# * Removed todo item: allow other comment directives for rst conversion
# * Added ability to use global rst style file _rststyle_._include_.tex
# * Added help text to that effect
# Chris Monson (2007-05-20):
# * Bumped version to 2.1.6
# * Changed default paper size for rst files
# * Added todo item: fix paper size for rst files
# * Added todo item: allow other comment directives for rst conversion
# Chris Monson (2007-04-02):
# * Bumped version to 2.1.5
# * Addressed Issue 7, incorrect .gpi.d generation in subdirectories
# Chris Monson (2007-03-28):
# * Bumped version to 2.1.4
# * Fixed syntax error in dot output
# Chris Monson (2007-03-01):
# * Bumped version to 2.1.3
# * Added reST to the included documentation
# * Fixed graphics and script generation to be settable in the
#     environment.
# Chris Monson (2007-02-23):
# * Bumped version to 2.1.2
# * Added the ability to generate .tex files from .rst files
# Chris Monson (2006-10-17):
# * Bumped version to 2.1.1
# * Fixed includes from subdirectories (sed-to-sed slash escape problem)
# Chris Monson (2006-10-05):
# * Bumped version to 2.1.0 (pretty serious new feature added)
# * New feature: bib files can now be anywhere on the BIBINPUTS path
# * New programs: kpsewhich (with tetex) and xargs (BSD)
# Chris Monson (2006-09-28):
# * Bumped version to 2.0.9
# * Added ability to parse more than one bibliography
# Chris Monson (2006-06-01):
# * Bumped version to 2.0.8
# * Added .vrb to the list of cleaned files
# Chris Monson (2006-04-26):
# * Bumped version to 2.0.7
# * Fixed so that clean-nographics does not remove .gpi.d files
# * Removed jpg -> eps hack (not working properly -- just pre-convert)
# * Fixed so that postscript grayscale can be done with BSD sed
# Chris Monson (2006-04-25):
# * Bumped version to 2.0.6
# * Fixed so that changed toc, lot, lof, or out causes a rebuild
# Chris Monson (2006-04-17):
# * Bumped version to 2.0.5
# * Added jpg -> eps conversion target
# Chris Monson (2006-04-12):
# * Bumped version to 2.0.4
# * Fixed BSD sed invocation to not use \| as a branch delimiter
# * Added a comment section on what is and is not allowed in BSD sed
# * Made paper size handling more robust while I was at it
# * Fixed postscript RGB grayscale to use a weighted average
# * Fixed postscript HSB grayscale to convert to RGB first
# * Fixed a problem with rebuilding .bbl files
# Chris Monson (2006-04-11):
# * Bumped version to 2.0.3
# * Fixed some BSD sed problems: can't use \n in substitutions
# Chris Monson (2006-04-10):
# * Bumped version to 2.0.2
# * Once again removed ability to create .tex files from scripts
# * \includeonly works again
# Chris Monson (2006-04-09):
# * Bumped version to 2.0.1
# * Fixed grayscale postscript handling to be more robust
# * Added ability to generate ._gray_. files from eps and eps.gz
# * Added ability to clean ._gray_.eps files created from .eps files
# Chris Monson (2006-04-07):
# * Bumped version to 2.0.0
# * Removed clunky ability to create included .tex files from scripts
# * Added note in the help about included tex scripting not working
# * Fixed the .eps generation to delete %.gpihead.make when finished
# * Abandoned designs to use shell variables to create sed scripts
# * Abandoned __default__.tex.sh idea: it causes recursion with %: .
# * Removed web page to-do.  All items are now complete.
# * Added better grayscale conversion for dot figures (direct ps fixup).
# * Include files can now be scripted (at the expense of \includeonly).
# * Updated dependency graph to contain better node names.
# Chris Monson (2006-04-06):
# * Bumped version to 2.0b3
# * Top level includes now fail if there is no rule to build them
# * A helpful message is printed when they do fail
# * Grayscale has been changed to be ._gray_, other phonies use _ now, too
# * Grayscale handling has been completed
# * Changed _include_stems target to _includes target.
# * Fixed _includes target to be useful by itself.
# * Removed the ability to specify clean and build targets at once
# * Verified that epsfig works fine with current code
# * Fixed included scripts so that they are added to the dep files
# * Fixed so that graphics includes don't happen if they aren't for gpi
# * Fixed dot output to allow grayscale.
# Chris Monson (2006-04-05):
# * Bumped version to 2.0b2
# * Removed automatic -gray output.  It needs fixing in a bad way.
# * Revamped dependency creation completely.
# * Fixed conditional inclusion to actually work (test.nobuild.d, test.d).
# * Fixed clean target to remove log targets
# * Added the 'monochrome' word for gray gpi output
# * Added a _check_gpi_files target that checks for common problems
# * Changed the _version target into the version target (no _)
# * Added better handling of grayscale files.  Use the .gray.pdf target.
# * Fixed testing for rebuilds
# Chris Monson (2006-04-04):
# * Bumped version to 2.0b1
# * Changed colorization of output
# * Made .auxbbl and .auxtex .make files secondary targets
# * Shortened and simplified the final latex invocation loop
# * Added version-specific output ($$i vs. $$$$i) in latex loop
# * Added a build message for the first .dvi run (Building .dvi (0))
# * Removed some build messages that most people don't care about.
# * Simplified procedure for user-set colors -- simple text specification
# * Fixed diff output to...not output.
# * Fixed rerun bug -- detect not only when preceded with LaTeX Warning
# * Sped up gpi plotting
# * Added error handling and colorized output for gpi failure
# * Documented color changing stuff.
# * Now sort the flattened aux file to avoid false recompilation needs
# * Added clean-nographics target
# * Don't remove self.dvi file if self.aux is missing in the log
# * Clarified some code.  Did some very minor adjusting.
# Chris Monson (2006-04-03):
# * Bumped version to 2.0a7
# * Added .dvi and .ps files as secondary files.
# * Fixed handling of multiple run detection when includeonly is in use.
# * Added code to flatten .aux files.
# * Added more files as .SECONDARY prerequisites to avoid recompilation.
# * Fixed the inputs generation to be much simpler and to use pipes.
# * Added the dependency graph directly into the makefile.
# * Changed flatten-aux to remove \@writefile \relax \newlabel, etc.
# * Undid pipe changes with sed usage (BSD sed doesn't know -f-).
# * Added a _check_programs target that tells you what your system has.
# * Fixed an error in colorization that made unnecessary errors appear
# * Added view targets.
# * Updated help text.
# * Augmented cookies so that .aux can trigger .bbl and .dvi rebuilds
# * Added more informative error handling for dvips and ps2pdf
# Chris Monson (2006-04-02):
# * Bumped version to 2.0a6
# * Added indirection to .bbl dependencies to avoid rebuilding .bbl files
# * Streamlined the diff invocation to eliminate an existence test
# * Removed special shell quote escape variables
# * Moved includes to a more prominent location
# * Fixed .inputs.make to not contain .aux files
# * Fixed embedding to use a file instead of always grepping.
# * Added *.make.temp to the list of cleanable files
# * Fixed Ruby.  It should now be supported properly.
# * Now differentiate between all, default, and buildable files.
# * Fixed to bail out on serious errors.
# * Revised the handling of includable files.  Still working on it.
# Chris Monson (2006-03-31):
# * Bumped version to 2.0a5
# * Fixed a bug with LaTeX error detection (there can be spaces)
# * Added .bbl support, simplifying everything and making it more correct
# * Refactored some tests that muddy the code
# * Did a little cleanup of some shell loops that can safely be make loops
# * Added support for graphviz .dot files
# * Made _all_programs output easier to read
# * Added the ruby support that has long been advertised
# * Font embedding was screwed up for PostScript -- now implicit
# * Changed the generation of -gray.gpi files to a single command
# * Changed any make-generated file that is not included from .d to .make
# Chris Monson (2006-03-30):
# * Bumped version to 2.0a4
# * Fixed a bug with very long graphics file names
# * Added a todo entry for epsfig support
# * Fixed a bug paper size bug: sometimes more than one entry appears
# * Fixed DVI build echoing to display the number instead of process ID
# * DVI files are now removed on first invocation if ANY file is missing
# * Added a simple grayscale approach: if a file ends with -gray.gpi, it
#     is created from the corresponding .gpi file with a special
#     comment ##GRAY in its header, which causes coloring to be
#     turned off.
# * Fixed a bug in the handling of .tex.sh files.  For some reason I had
#     neglected to define file stems for scripted output.
# * Removed a trailing ; from the %.graphics dependencies
# * Added dvips embedding (I think it works, anyway)
# Chris Monson (2006-03-29):
# * Bumped version to 2.0a3
# * Fixed error in make 3.79 with MAKEFILE_LIST usage
# * Added the presumed filename to the _version output
# * Added a vim macro for converting sed scripts to make commands
# * Added gpi dependency support (plotting external files and loading gpi)
# * Allow .gpi files to be ignored if called .include.gpi or .nobuild.gpi
# * Fixed sed invocations where \+ was used.  BSD sed uses \{1,\}.
# Chris Monson (2006-03-28):
# * Bumped version to 2.0a2
# * Added SHELL_DEBUG and VERBOSE options
# * Changed the default shell back to /bin/sh (unset, in other words)
# * Moved .PHONY declarations closer to their targets
# * Moved help text into its own define block to obtain better formatting
# * Removed need for double-entry when adding a new program invocation
# * Moved .SECONDARY declaration closer to its relevant occurrence
# * Commented things more heavily
# * Added help text about setting terminal and output in gnuplot
# * Created more fine-grained clean targets
# * Added a %.graphics target that generates all of %'s graphics
# * Killed backward-compatible graphics generation (e.g., eps.gpi=gpi.eps)
# * For now, we're just GPL 2, not 3.  Maybe it will change later
# * Made the version and svninfo into variables
# Chris Monson (2006-03-27):
# * Bumped version to 2.0a1
# * Huge, sweeping changes -- automatic dependencies
#

# IMPORTANT!
#
# When adding to the following list, do not introduce any blank lines.  The
# list is extracted for documentation using sed and is terminated by a blank
# line.
#
# EXTERNAL PROGRAMS:
# = ESSENTIAL PROGRAMS =
# == Basic Shell Utilities ==
CAT		?= cat
CP		?= cp -f
DIFF		?= diff
ECHO		?= echo
EGREP		?= egrep
ENV		?= env
EXPR		?= expr
MV		?= mv -f
SED		?= sed
SORT		?= sort
TOUCH		?= touch
UNIQ		?= uniq
WHICH		?= which
XARGS		?= xargs
SLEEP		?= sleep
# == LaTeX (tetex-provided) ==
BIBTEX		?= bibtex
DVIPS		?= dvips
LATEX		?= latex
PDFLATEX	?= pdflatex
XELATEX		?= xelatex
EPSTOPDF	?= epstopdf
MAKEINDEX	?= makeindex
XINDY		?= xindy
KPSEWHICH	?= kpsewhich
GS		?= gs
# = OPTIONAL PROGRAMS =
# == For MikTex under Cygwin, to get path names right
CYGPATH		?= cygpath
# == Makefile Color Output ==
TPUT		?= tput
# == TeX Generation ==
PERL		?= perl
PYTHON		?= python
RST2LATEX	?= rst2latex.py
# == EPS Generation ==
CONVERT		?= convert	# ImageMagick
DOT		?= dot		# GraphViz
DOT2TEX		?= dot2tex	# dot2tex - add options (not -o) as needed
FIG2DEV		?= fig2dev	# XFig
GNUPLOT		?= gnuplot	# GNUplot
INKSCAPE	?= inkscape	# Inkscape (svg support)
XMGRACE		?= xmgrace	# XMgrace
PNGTOPNM	?= pngtopnm	# From NetPBM - step 1 for png -> eps
PPMTOPGM	?= ppmtopgm	# From NetPBM - (gray) step 2 for png -> eps
PNMTOPS		?= pnmtops	# From NetPBM - step 3 for png -> eps
GUNZIP		?= gunzip	# GZipped EPS
# == Beamer Enlarged Output ==
PSNUP		?= psnup
# == Viewing Stuff ==
VIEW_POSTSCRIPT	?= gv
VIEW_PDF	?= xpdf
VIEW_GRAPHICS	?= display

# Xindy glossaries
XINDYLANG	?= english
XINDYENC	?= utf8

# If cygpath is present, then we create a path-norm function that uses it,
# otherwise the function is just a no-op.  Issue 112 has details.
USE_CYGPATH := $(if $(shell $(WHICH) $(CYGPATH) 2>/dev/null),yes,)

# $(call get-cygpath,<path>)
define get-cygpath
$(shell $(CYGPATH) -u "$(shell $(CYGPATH) -s -w $1)")
endef

define path-norm
$(if $(USE_CYGPATH),$(call get-cygpath,$1),$1)
endef

# Command options for embedding fonts and postscript->pdf conversion
PS_EMBED_OPTIONS	?= -dPDFSETTINGS=/printer -dEmbedAllFonts=true -dSubsetFonts=true -dMaxSubsetPct=100
PS_COMPATIBILITY	?= 1.4

# If set to something, will cause temporary files to not be deleted immediately
KEEP_TEMP	?=

# Defaults for GPI
DEFAULT_GPI_EPS_FONTSIZE	?= 22
DEFAULT_GPI_PDF_FONTSIZE	?= 12

# Style file for ReST
RST_STYLE_FILE			?= $(wildcard _rststyle_._include_.tex)

# This ensures that even when echo is a shell builtin, we still use the binary
# (the builtin doesn't always understand -n)
FIXED_ECHO	:= $(if $(findstring -n,$(shell $(ECHO) -n)),$(shell which echo),$(ECHO))
ECHO		:= $(if $(FIXED_ECHO),$(FIXED_ECHO),$(ECHO))

define determine-gnuplot-output-extension
$(if $(shell $(WHICH) $(GNUPLOT) 2>/dev/null),
     $(if $(findstring unknown or ambiguous, $(shell $(GNUPLOT) -e "set terminal pdf" 2>&1)),
	  eps, pdf),
     none)
endef

GNUPLOT_OUTPUT_EXTENSION	?= $(strip $(call determine-gnuplot-output-extension))

# Internal code should use this because of :=.  This means that the potentially
# expensive script invocation used to determine whether pdf is available will
# only be run once.
GPI_OUTPUT_EXTENSION := $(strip $(GNUPLOT_OUTPUT_EXTENSION))

# Note, if the terminal *does* understand fsize, then we expect this call to
# create a specific error here: "fsize: expecting font size".  Otherwise, we
# assume that fsize is not understood.
GPI_FSIZE_SYNTAX := $(strip \
$(if \
  $(filter pdf,$(GPI_OUTPUT_EXTENSION)),\
  $(if \
    $(findstring fsize: expecting font size,$(shell $(GNUPLOT) -e "set terminal pdf fsize" 2>&1)),\
    fsize FONTSIZE,\
    font ",FONTSIZE"),\
  FONTSIZE))

# Directory into which we place "binaries" if it exists.
# Note that this can be changed on the commandline or in Makefile.ini:
#
# Command line:
#   make BINARY_TARGET_DIR=$HOME/pdfs myfile.pdf
#
# Also, you can specify a relative directory (relative to the Makefile):
#   make BINARY_TARGET_DIR=pdfs myfile.pdf
#
# Or, you can use Makefile.ini:
#
#   BINARY_TARGET_DIR := $(HOME)/bin_out
#
BINARY_TARGET_DIR	?= _out_

RESTARTS		:= $(if $(MAKE_RESTARTS),$(MAKE_RESTARTS),0)
# SH NOTES
#
# On some systems, /bin/sh, which is the default shell, is not linked to
# /bin/bash.  While bash is supposed to be sh-compatible when invoked as sh, it
# just isn't.  This section details some of the things you have to stay away
# from to remain sh-compatible.
#
#	* File pattern expansion does not work for {}
#	* [ "$x" = "$y" ] has to be [ x"$x" x"$y" ]
#	* &> for stderr redirection doesn't work, use 2>&1 instead
#
# BSD SED NOTES
#
# BSD SED is not very nice compared to GNU sed, but it is the most
# commonly-invoked sed on Macs (being based on BSD), so we have to cater to
# it or require people to install GNU sed.  It seems like the GNU
# requirement isn't too bad since this makefile is really a GNU makefile,
# but apparently GNU sed is much less common than GNU make in general, so
# I'm supporting it here.
#
# Sad experience has taught me the following about BSD sed:
#
# 	* \+ is not understood to mean \{1,\}
# 	* \| is meaningless (does not branch)
# 	* \n cannot be used as a substitution character
# 	* ? does not mean \{0,1\}, but is literal
# 	* a\ works, but only reliably for a single line if subsequent lines
# 		have forward slashes in them (as is the case in postscript)
#
# For more info (on the Mac) you can consult
#
# man -M /usr/share/man re_format
#
# And look for the word "Obsolete" near the bottom.

#
# EXTERNAL PROGRAM DOCUMENTATION SCRIPT
#

# $(call output-all-programs,[<output file>])
define output-all-programs
	[ -f '$(this_file)' ] && \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*EXTERNAL PROGRAMS:/,/^$$/!d' \
		-e '/EXTERNAL PROGRAMS/d' \
		-e '/^$$/d' \
		-e '/^[[:space:]]*#/i\ '\
		-e 's/^[[:space:]]*#[[:space:]][^=]*//' \
		$(this_file) $(if $1,> '$1',) || \
	$(ECHO) "Cannot determine the name of this makefile."
endef

# If they misspell gray, it should still work.
GRAY	?= $(call get-default,$(GREY),)

#
# Utility Functions and Definitions
#

# Don't call this directly - it is here to avoid calling wildcard more than
# once in remove-files.
remove-files-helper	= $(if $1,$(RM) $1,$(sh_true))

# $(call remove-files,file1 file2)
remove-files		= $(call remove-files-helper,$(wildcard $1))

# Removes all cleanable files in the given list
# $(call clean-files,file1 file2 file3 ...)
# Works exactly like remove-files, but filters out files in $(neverclean)
clean-files		= \
	$(call remove-files-helper,$(call cleanable-files,$(wildcard $1)))

# Outputs all generated files to STDOUT, along with some others that are
# created by these (e.g., .idx files end up producing .ilg and .ind files).
# Discovered by reading *.fls OUTPUT lines and producing corresponding .ind
# filenames as needed.
#
# $(call get-generated-names,<source recorder file (*.fls)>)
define get-generated-names
[ -f '$1' ] && \
$(SED) \
	-e '/^OUTPUT /{' \
	-e '  s///' \
	-e '  p' \
	-e '  s/\.idx/\.ind/p' \
	-e '  s/\.ind/\.ilg/p' \
	-e '}' \
	-e 'd' \
	'$1' \
| $(SORT) | $(UNIQ)
endef

# This removes files without checking whether they are there or not.  This
# sometimes has to be used when the file is created by a series of shell
# commands, but there ends up being a race condition: make doesn't know about
# the file generation as quickly as the system does, so $(wildcard ...) doesn't
# work right.  Blech.
# $(call remove-temporary-files,filenames)
remove-temporary-files	= $(if $(KEEP_TEMP),:,$(if $1,$(RM) $1,:))

# Create an identifier from a file name
# $(call cleanse-filename,filename)
cleanse-filename	= $(subst .,_,$(subst /,__,$1))

# Escape dots
# $(call escape-fname-regex,str)
escape-fname-regex	= $(subst /,\\/,$(subst .,\\.,$1))

# Test that a file exists
# $(call test-exists,file)
test-exists		= [ -e '$1' ]

# $(call move-files,source,destination)
move-if-exists		= $(call test-exists,$1) && $(MV) '$1' '$2'

# Copy file1 to file2 only if file2 doesn't exist or they are different
# $(call copy-if-different,sfile,dfile)
copy-if-different	= $(call test-different,$1,$2) && $(CP) '$1' '$2'
copy-if-exists		= $(call test-exists,$1) && $(CP) '$1' '$2'
move-if-different	= $(call test-different,$1,$2) && $(MV) '$1' '$2'
replace-if-different-and-remove	= \
	$(call test-different,$1,$2) \
	&& $(MV) '$1' '$2' \
	|| $(call remove-files,'$1')

# Note that $(DIFF) returns success when the files are the SAME....
# $(call test-different,sfile,dfile)
test-different		= ! $(DIFF) -q '$1' '$2' >/dev/null 2>&1
test-exists-and-different	= \
	$(call test-exists,$2) && $(call test-different,$1,$2)

# Return value 1, or value 2 if value 1 is empty
# $(call get-default,<possibly empty arg>,<default value if empty>)
get-default	= $(if $1,$1,$2)

# Copy a file and log what's going on
# $(call copy-with-logging,<source>,<target>)
define copy-with-logging
if [ -d '$2/' ]; then \
	if $(CP) '$1' '$2/'; then \
		$(ECHO) "$(C_INFO)Copied '$1' to '$2/'$(C_RESET)"; \
	else \
		$(ECHO) "$(C_ERROR)Failed to copy '$1' to '$2/'$(C_RESET)"; \
	fi; \
fi
endef

# Gives a reassuring message about the failure to find include files
# $(call include-message,<list of include files>)
define include-message
$(strip \
$(if $(filter-out $(wildcard $1),$1),\
	$(shell $(ECHO) \
	"$(C_INFO)NOTE: You may ignore warnings about the"\
	"following files:" >&2;\
	$(ECHO) >&2; \
	$(foreach s,$(filter-out $(wildcard $1),$1),$(ECHO) '     $s' >&2;)\
	$(ECHO) "$(C_RESET)" >&2)
))
endef
# Characters that are hard to specify in certain places
space		:= $(empty) $(empty)
colon		:= \:
comma		:= ,

# Useful shell definitions
sh_true		:= :
sh_false	:= ! :

# Clear out the standard interfering make suffixes
.SUFFIXES:

# Turn off forceful rm (RM is usually mapped to rm -f)
ifdef SAFE_RM
RM	:= rm
endif

# Turn command echoing back on with VERBOSE=1
ifndef VERBOSE
QUIET	:= @
endif

# Turn on shell debugging with SHELL_DEBUG=1
# (EVERYTHING is echoed, even $(shell ...) invocations)
ifdef SHELL_DEBUG
SHELL	+= -x
endif

# Get the name of this makefile (always right in 3.80, often right in 3.79)
# This is only really used for documentation, so it isn't too serious.
ifdef MAKEFILE_LIST
this_file	:= $(word $(words $(MAKEFILE_LIST)),$(MAKEFILE_LIST))
else
this_file	:= $(wildcard GNUmakefile makefile Makefile)
endif

# Terminal color definitions

REAL_TPUT 	:= $(if $(NO_COLOR),,$(shell $(WHICH) $(TPUT)))

# $(call get-term-code,codeinfo)
# e.g.,
# $(call get-term-code,setaf 0)
get-term-code = $(if $(REAL_TPUT),$(shell $(REAL_TPUT) $1),)

black	:= $(call get-term-code,setaf 0)
red	:= $(call get-term-code,setaf 1)
green	:= $(call get-term-code,setaf 2)
yellow	:= $(call get-term-code,setaf 3)
blue	:= $(call get-term-code,setaf 4)
magenta	:= $(call get-term-code,setaf 5)
cyan	:= $(call get-term-code,setaf 6)
white	:= $(call get-term-code,setaf 7)
bold	:= $(call get-term-code,bold)
uline	:= $(call get-term-code,smul)
reset	:= $(call get-term-code,sgr0)

#
# User-settable definitions
#
LATEX_COLOR_WARNING	?= magenta
LATEX_COLOR_ERROR	?= red
LATEX_COLOR_INFO	?= green
LATEX_COLOR_UNDERFULL	?= magenta
LATEX_COLOR_OVERFULL	?= red bold
LATEX_COLOR_PAGES	?= bold
LATEX_COLOR_BUILD	?= cyan
LATEX_COLOR_GRAPHIC	?= yellow
LATEX_COLOR_DEP		?= green
LATEX_COLOR_SUCCESS	?= green bold
LATEX_COLOR_FAILURE	?= red bold

# Gets the real color from a simple textual definition like those above
# $(call get-color,ALL_CAPS_COLOR_NAME)
# e.g., $(call get-color,WARNING)
get-color	= $(subst $(space),,$(foreach c,$(LATEX_COLOR_$1),$($c)))

#
# STANDARD COLORS
#
C_WARNING	:= $(call get-color,WARNING)
C_ERROR		:= $(call get-color,ERROR)
C_INFO		:= $(call get-color,INFO)
C_UNDERFULL	:= $(call get-color,UNDERFULL)
C_OVERFULL	:= $(call get-color,OVERFULL)
C_PAGES		:= $(call get-color,PAGES)
C_BUILD		:= $(call get-color,BUILD)
C_GRAPHIC	:= $(call get-color,GRAPHIC)
C_DEP		:= $(call get-color,DEP)
C_SUCCESS	:= $(call get-color,SUCCESS)
C_FAILURE	:= $(call get-color,FAILURE)
C_RESET		:= $(reset)

#
# PRE-BUILD TESTS
#

# Check that clean targets are not combined with other targets (weird things
# happen, and it's not easy to fix them)
hascleangoals	:= $(if $(sort $(filter clean clean-%,$(MAKECMDGOALS))),1)
hasbuildgoals	:= $(if $(sort $(filter-out clean clean-%,$(MAKECMDGOALS))),1)
ifneq "$(hasbuildgoals)" ""
ifneq "$(hascleangoals)" ""
$(error $(C_ERROR)Clean and build targets specified together$(C_RESET)))
endif
endif

#
# VARIABLE DECLARATIONS
#

# Names of sed scripts that morph gnuplot files -- only the first found is used
GNUPLOT_SED	:= global-gpi.sed gnuplot.sed
GNUPLOT_GLOBAL	:= global._include_.gpi gnuplot.global

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
default_graphic_extension	?= eps
latex_build_program		?= $(LATEX)
build_target_extension		?= dvi
hyperref_driver_pattern		?= hdvips
hyperref_driver_error		?= Using dvips: specify ps2pdf in the hyperref options.
endif

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
default_graphic_extension	?= pdf
latex_build_program		?= $(PDFLATEX)
build_target_extension		?= pdf
hyperref_driver_pattern		?= hpdf.*
hyperref_driver_error		?= Using pdflatex: specify pdftex in the hyperref options (or leave it blank).
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
default_graphic_extension	?= pdf
latex_build_program		?= $(XELATEX)
build_target_extension		?= pdf
hyperref_driver_pattern		?= hdvipdf.*
hyperref_driver_error		?= Using pdflatex: specify pdftex in the hyperref options (or leave it blank).
endif

# Files of interest
all_files.tex		?= $(wildcard *.tex)
all_files.tex.sh	?= $(wildcard *.tex.sh)
all_files.tex.pl	?= $(wildcard *.tex.pl)
all_files.tex.py	?= $(wildcard *.tex.py)
all_files.rst		?= $(wildcard *.rst)
all_files.fig		?= $(wildcard *.fig)
all_files.gpi		?= $(wildcard *.gpi)
all_files.dot		?= $(wildcard *.dot)
all_files.xvg		?= $(wildcard *.xvg)
all_files.svg		?= $(wildcard *.svg)
all_files.png		?= $(wildcard *.png)
all_files.jpg		?= $(wildcard *.jpg)
all_files.jpeg		?= $(wildcard *.jpeg)
all_files.eps.gz	?= $(wildcard *.eps.gz)
all_files.eps		?= $(wildcard *.eps)

# Utility function for obtaining all files not specified in $(neverclean)
# $(call cleanable-files,file1 file2 file3 ...)
# Returns the list of files that is not in $(wildcard $(neverclean))
cleanable-files = $(filter-out $(wildcard $(neverclean)), $1)

# Utility function for getting all .$1 files that are to be ignored
#  * files listed in $(includes.$1)
#  * files not listed in $(onlysources.$1) if it is defined
ignore_files = \
  $(includes.$1) \
  $(if $(onlysources.$1),$(filter-out $(onlysources.$1), $(all_files.$1)))

# Patterns to never be allowed as source targets
ignore_patterns	:= %._include_

# Patterns allowed as source targets but not included in 'all' builds
nodefault_patterns := %._nobuild_ $(ignore_patterns)

# Utility function for getting targets suitable building
# $(call filter-buildable,suffix)
filter-buildable	= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(ignore_patterns)),$(all_files.$1))

# Utility function for getting targets suitable for 'all' builds
# $(call filter-default,suffix)
filter-default		= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(nodefault_patterns)),$(all_files.$1))

# Top level sources that can be built even when they are not by default
files.tex	:= $(call filter-buildable,tex)
files.tex.sh	:= $(call filter-buildable,tex.sh)
files.tex.pl	:= $(call filter-buildable,tex.pl)
files.tex.py	:= $(call filter-buildable,tex.py)
files.rst	:= $(call filter-buildable,rst)
files.gpi	:= $(call filter-buildable,gpi)
files.dot	:= $(call filter-buildable,dot)
files.fig	:= $(call filter-buildable,fig)
files.xvg	:= $(call filter-buildable,xvg)
files.svg	:= $(call filter-buildable,svg)
files.png	:= $(call filter-buildable,png)
files.jpg	:= $(call filter-buildable,jpg)
files.jpeg	:= $(call filter-buildable,jpeg)
files.eps.gz	:= $(call filter-buildable,eps.gz)
files.eps	:= $(call filter-buildable,eps)

# Make all pstex targets secondary.  The pstex_t target requires the pstex
# target, and nothing else really depends on it, so it often gets deleted.
# This avoids that by allowing *all* fig files to be pstex targets, which is
# perfectly valid and causes no problems even if they're going to become eps
# files in the end.
.SECONDARY:	$(patsubst %.fig,%.pstex,$(files.fig))

# Top level sources that are built by default targets
default_files.tex	:= $(call filter-default,tex)
default_files.tex.sh	:= $(call filter-default,tex.sh)
default_files.tex.pl	:= $(call filter-default,tex.pl)
default_files.tex.py	:= $(call filter-default,tex.py)
default_files.rst	:= $(call filter-default,rst)
default_files.gpi	:= $(call filter-default,gpi)
default_files.dot	:= $(call filter-default,dot)
default_files.fig	:= $(call filter-default,fig)
default_files.xvg	:= $(call filter-default,xvg)
default_files.svg	:= $(call filter-default,svg)
default_files.png	:= $(call filter-default,png)
default_files.jpg	:= $(call filter-default,jpg)
default_files.jpeg	:= $(call filter-default,jpeg)
default_files.eps.gz	:= $(call filter-default,eps.gz)
default_files.eps	:= $(call filter-default,eps)

# Utility function for creating larger lists of files
# $(call concat-files,suffixes,[prefix])
concat-files	= $(foreach s,$1,$($(if $2,$2_,)files.$s))

# Useful file groupings
all_files_source	:= $(call concat-files,tex,all)
all_files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst,all)

.PHONY: $(all_files_scripts)

default_files_source	:= $(call concat-files,tex,default)
default_files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst,default)

files_source	:= $(call concat-files,tex)
files_scripts	:= $(call concat-files,tex.sh tex.pl tex.py rst)

# Utility function for obtaining stems
# $(call get-stems,suffix,[prefix])
get-stems	= $(sort $($(if $2,$2_,)files.$1:%.$1=%))

# List of all stems (including ._include_ and ._nobuild_ file stems)
all_stems.tex		:= $(call get-stems,tex,all)
all_stems.tex.sh	:= $(call get-stems,tex.sh,all)
all_stems.tex.pl	:= $(call get-stems,tex.pl,all)
all_stems.tex.py	:= $(call get-stems,tex.py,all)
all_stems.rst		:= $(call get-stems,rst,all)
all_stems.fig		:= $(call get-stems,fig,all)
all_stems.gpi		:= $(call get-stems,gpi,all)
all_stems.dot		:= $(call get-stems,dot,all)
all_stems.xvg		:= $(call get-stems,xvg,all)
all_stems.svg		:= $(call get-stems,svg,all)
all_stems.png		:= $(call get-stems,png,all)
all_stems.jpg		:= $(call get-stems,jpg,all)
all_stems.jpeg		:= $(call get-stems,jpeg,all)
all_stems.eps.gz	:= $(call get-stems,eps.gz,all)
all_stems.eps		:= $(call get-stems,eps,all)

# List of all default stems (all default PDF targets):
default_stems.tex		:= $(call get-stems,tex,default)
default_stems.tex.sh		:= $(call get-stems,tex.sh,default)
default_stems.tex.pl		:= $(call get-stems,tex.pl,default)
default_stems.tex.py		:= $(call get-stems,tex.py,default)
default_stems.rst		:= $(call get-stems,rst,default)
default_stems.fig		:= $(call get-stems,fig,default)
default_stems.gpi		:= $(call get-stems,gpi,default)
default_stems.dot		:= $(call get-stems,dot,default)
default_stems.xvg		:= $(call get-stems,xvg,default)
default_stems.svg		:= $(call get-stems,svg,default)
default_stems.png		:= $(call get-stems,png,default)
default_stems.jpg		:= $(call get-stems,jpg,default)
default_stems.jpeg		:= $(call get-stems,jpeg,default)
default_stems.eps.gz		:= $(call get-stems,eps.gz,default)
default_stems.eps		:= $(call get-stems,eps,default)

# List of all stems (all possible bare PDF targets created here):
stems.tex		:= $(call get-stems,tex)
stems.tex.sh		:= $(call get-stems,tex.sh)
stems.tex.pl		:= $(call get-stems,tex.pl)
stems.tex.py		:= $(call get-stems,tex.py)
stems.rst		:= $(call get-stems,rst)
stems.fig		:= $(call get-stems,fig)
stems.gpi		:= $(call get-stems,gpi)
stems.dot		:= $(call get-stems,dot)
stems.xvg		:= $(call get-stems,xvg)
stems.svg		:= $(call get-stems,svg)
stems.png		:= $(call get-stems,png)
stems.jpg		:= $(call get-stems,jpg)
stems.jpeg		:= $(call get-stems,jpeg)
stems.eps.gz		:= $(call get-stems,eps.gz)
stems.eps		:= $(call get-stems,eps)

# Utility function for creating larger lists of stems
# $(call concat-stems,suffixes,[prefix])
concat-stems	= $(sort $(foreach s,$1,$($(if $2,$2_,)stems.$s)))

# The most likely to be source but not finished product go first
graphic_source_extensions	:= fig \
				   gpi \
				   xvg \
				   svg \
				   dot \
				   eps.gz

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
graphic_source_extensions	+= png jpg jpeg
graphic_target_extensions	:= eps ps
endif

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
graphic_source_extensions	+= eps
graphic_target_extensions	:= pdf png jpg jpeg mps tif
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
graphic_source_extensions	+= eps
graphic_target_extensions	:= pdf png jpg jpeg mps tif
endif

all_stems_source	:= $(call concat-stems,tex,all)
all_stems_script	:= $(call concat-stems,tex.sh tex.pl tex.py rst,all)
all_stems_graphic	:= $(call concat-stems,$(graphic_source_extensions),all)
all_stems_ss		:= $(sort $(all_stems_source) $(all_stems_script))
all_stems_sg		:= $(sort $(all_stems_script))
all_stems_ssg		:= $(sort $(all_stems_ss))

default_stems_source	:= $(call concat-stems,tex,default)
default_stems_script	:= $(call concat-stems,tex.sh tex.pl tex.py rst,default)
default_stems_ss	:= $(sort $(default_stems_source) $(default_stems_script))
default_stems_sg	:= $(sort $(default_stems_script))
default_stems_ssg	:= $(sort $(default_stems_ss))

stems_source		:= $(call concat-stems,tex)
stems_script		:= $(call concat-stems,tex.sh tex.pl tex.py rst)
stems_graphic		:= $(call concat-stems,$(graphic_source_extensions))
stems_gg		:= $(sort $(stems_graphic))
stems_ss		:= $(sort $(stems_source) $(stems_script))
stems_sg		:= $(sort $(stems_script))
stems_ssg		:= $(sort $(stems_ss))

# Calculate names that can generate the need for an include file.  We can't
# really do this with patterns because it's too easy to screw up, so we create
# an exhaustive list.
allowed_source_suffixes	:= \
	pdf \
	ps \
	dvi \
	ind \
	nls \
	bbl \
	aux \
	aux.make \
	d \
	auxbbl.make \
	_graphics \
	_show
allowed_source_patterns		:= $(addprefix %.,$(allowed_source_suffixes))

allowed_graphic_suffixes	:= \
	pdf \
	eps \
	gpihead.make \
	gpi.d
allowed_graphic_patterns	:= $(addprefix %.,$(allowed_graphic_suffixes))

# All targets allowed to build documents
allowed_source_targets	:= \
	$(foreach suff,$(allowed_source_suffixes),\
	$(addsuffix .$(suff),$(stems_ssg)))

# All targets allowed to build graphics
allowed_graphic_targets	:= \
	$(foreach suff,$(allowed_graphic_suffixes),\
	$(addsuffix .$(suff),$(stems_gg)))

# All targets that build multiple documents (like 'all')
allowed_batch_source_targets	:= \
	all \
	all-pdf \
	all-ps \
	all-dvi \
	all-bbl \
	all-ind \
	all-gls \
	all-nls \
	show

# All targets that build multiple graphics (independent of document)
allowed_batch_graphic_targets	:= \
	all-graphics \
	all-pstex \
	all-dot2tex \
	show-graphics

# Now we figure out which stuff is available as a make target for THIS RUN.
real_goals	:= $(call get-default,$(filter-out _includes,$(MAKECMDGOALS)),\
			all)

specified_source_targets	:= $(strip \
	$(filter $(allowed_source_targets) $(stems_ssg),$(real_goals)) \
	)

specified_batch_source_targets	:= $(strip \
	$(filter $(allowed_batch_source_targets),$(real_goals)) \
	)

specified_graphic_targets	:= $(strip \
	$(filter $(allowed_graphic_targets),$(real_goals)) \
	)

specified_batch_graphic_targets	:= $(strip \
	$(filter $(allowed_batch_graphic_targets),$(real_goals)) \
	)

specified_gpi_targets	:= $(patsubst %.gpi,%.$(default_graphic_extension),\
	$(filter $(patsubst %.$(default_graphic_extension),%.gpi,$(specified_graphic_targets)),\
		$(all_files.gpi)) \
	)

# Determine which .d files need including from the information gained above.
# This is done by first checking whether a batch target exists.  If it does,
# then all *default* stems are used to create possible includes (nobuild need
# not apply for batch status).  If no batch targets exist, then the individual
# targets are considered and appropriate includes are taken from them.
source_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_source_targets),\
		$(default_stems_ss),\
		$(foreach t,$(specified_source_targets),\
		$(foreach p,$(allowed_source_patterns),\
			$(patsubst $p,%,$(filter $p $(stems_ssg),$t)) \
		)) \
	))

# Determine which .gpi.d files are needed using the above information.  We
# first check whether a batch target is specified, then check individual
# graphics that may have been specified.
graphic_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_graphic_targets),\
		$(default_stems.gpi),\
		$(foreach t,$(specified_gpi_targets),\
		$(foreach p,$(allowed_graphic_patterns),\
			$(patsubst $p,%,$(filter $p,$t)) \
		)) \
	))

# All dependencies for the 'all' targets
all_pdf_targets		:= $(addsuffix .pdf,$(stems_ssg))
all_ps_targets		:= $(addsuffix .ps,$(stems_ssg))
all_dvi_targets		:= $(addsuffix .dvi,$(stems_ssg))
all_tex_targets		:= $(addsuffix .tex,$(stems_sg))
all_d_targets		:= $(addsuffix .d,$(stems_ssg))
all_graphics_targets	:= $(addsuffix .$(default_graphic_extension),$(stems_gg))
all_pstex_targets	:= $(addsuffix .pstex_t,$(stems.fig))
all_dot2tex_targets	:= $(addsuffix .dot_t,$(stems.dot))

all_known_graphics	:= $(sort $(all_graphics_targets) $(wildcard *.$(default_graphic_extension)))

default_pdf_targets	:= $(addsuffix .pdf,$(default_stems_ss))

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
default_ps_targets	:= $(addsuffix .ps,$(default_stems_ss))
default_dvi_targets	:= $(addsuffix .dvi,$(default_stems_ss))
pre_pdf_extensions	:= dvi ps
endif

# Extensions generated by LaTeX invocation that can be removed when complete
rm_ext		:= \
	log *.log aux $(pre_pdf_extensions) pdf blg bbl out nav snm toc lof lot lol pfg \
	fls vrb idx ind ilg glg glo gls lox nls nlo nlg brf mtc maf brf ist
backup_patterns	:= *~ *.bak *.backup body.tmp head.tmp

graph_stem	:= _graph

# All LaTeX-generated files that can be safely removed

rm_tex := \
	$(foreach e,$(rm_ext),$(addsuffix .$e,$(all_stems_source))) \
	$(foreach e,$(rm_ext) tex,$(addsuffix .$e,$(all_stems_sg))) \
	$(addsuffix .log,$(all_ps_targets) $(all_pdf_targets)) \
	$(addsuffix .*.log,$(stems_graphic))

# These are the files that will affect .gpi transformation for all .gpi files.
#
# Use only the first one found.  Backward compatible values are at the end.
# Note that we use foreach, even though wildcard also returns a list, to ensure
# that the order in the uppercase variables is preserved.  Directory listings
# provide no such guarantee, so we avoid relying on them.
gpi_sed		:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_SED),$(wildcard $f))))
gpi_global	:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_GLOBAL),$(wildcard $f))))

#
# Functions used in generating output
#

# Outputs all source dependencies to stdout.  The first argument is the file to
# be parsed, the second is a list of files that will show up as dependencies in
# the new .d file created here.
#
# $(call get-inputs,<parsed file>,<target files>)
define get-inputs
$(SED) \
-e '/^INPUT/!d' \
-e 's!^INPUT \(\./\)\{0,1\}!!' \
-e 's/[[:space:]]/\\ /g' \
-e 's/\(.*\)\.aux$$/\1.tex/' \
-e '/\.tex$$/b addtargets' \
-e '/\.cls$$/b addtargets' \
-e '/\.sty$$/b addtargets' \
-e '/\.pstex_t$$/b addtargets' \
-e '/\.dot_t$$/b addtargets' \
-e 'd' \
-e ':addtargets' \
-e 's!.*!$2: $$(call path-norm,&)!' \
'$1' | $(SORT) | $(UNIQ)
endef

# $(call get-missing-inputs,<log file>,<target files>)
define get-missing-inputs
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^! LaTeX Error: File `/{' \
-e '  b needtwomore' \
-e '}' \
-e '/^::0::\(.*\)/{' \
-e '  s//\1/' \
-e '  /Default extension: /!d' \
-e '  s/.*File `\([^'"'"']*\)'"'"' not found.*/\1/' \
-e '  s/[[:cntrl:]]//' \
-e '  /\.tex/!s/$$/.tex/' \
-e '  s/[[:space:]]/\\ /g' \
-e '  h' \
-e '  s/.*/# MISSING input "&" - (presence of comment affects build)/' \
-e '  p' \
-e '  s/.*//' \
-e '  x' \
-e '  s!^.*!$2: $$(call path-norm,&)!' \
-e '  p' \
-e '}' \
-e 'd' \
'$1' | $(SORT) | $(UNIQ)
endef

# Get source file for specified graphics stem.
#
# $(call graphics-source,<stem>)
define graphics-source
$(strip $(firstword \
	$(wildcard \
		$(addprefix $1.,\
			$(graphic_source_extensions))) \
	$1 \
))
endef

# Get the target file for the specified graphics file/stem
#
# $(call graphics-target,<stem>)
define graphics-target
$(strip $(if 	$(filter $(addprefix %.,$(graphic_target_extensions)),$1), $1,
	$(firstword $(patsubst $(addprefix %.,$(graphic_source_extensions) $(graphic_target_extensions)), %, $1).$(default_graphic_extension) $1.$(default_graphic_extension))))
endef

# Outputs all of the graphical dependencies to stdout.  The first argument is
# the stem of the source file being built, the second is a list of suffixes
# that will show up as dependencies in the generated .d file.
#
# Note that we try to escape spaces in filenames where possible.  We have to do
# it with three backslashes so that as the name percolates through the makefile
# it eventually ends up with the proper escaping when the build rule is found.
# Ugly, but it appears to work.  Note that graphicx doesn't allow filenames
# with spaces, so this could in many ways be moot unless you're using something
# like grffile.
#
# For pdflatex, we really need the missing file to be specified without an
# extension, otherwise compilation barfs on the first missing file.  Truly
# annoying, but there you have it.
#
# It turns out that the graphics errors, although they have lines with empty
# space, are only made of two paragraphs.  So, we just use some sed magic to
# get everything into paragraphs, detect when it's a paragraph that interests
# us, and double it up.  Then we get the filename only if we're missing
# extensions (a sign that it's graphicx complaining).
#
# $(call get-graphics,<target file stem>)
#.log,$(addprefix $*.,d $(build_target_extension) _graphics)
define get-graphics
$(SED) \
-e '/^File: \(.*\) Graphic file (type [^)]*)/{' \
-e '  s//\1/' \
-e '  b addtargets' \
-e '}' \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^[^[:cntrl:]:]*:[[:digit:]]\{1,\}: LaTeX Error: File `/{' \
-e '  s/\n//g' \
-e '  b needonemore' \
-e '}' \
-e '/^::0::.*: LaTeX Error: File `/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/\n\{1,\}/ /g' \
-e '  s/[[:space:]]\{1,\}/ /g' \
-e '  s/^.*File `//' \
-e '  s/'"'"' not found\..*extensions: \([^[:space:]]*\).*/::::\1/' \
-e '  h' \
-e '  s/\(.*\)::::\(.*\)/# MISSING stem "\1" - allowed extensions are "\2" - leave comment here - it affects the build/' \
-e '  p' \
-e '  g' \
-e '  s/::::.*//' \
-e '  b addtargets' \
-e '}' \
-e 'd' \
-e ':addtargets' \
-e 's/[[:space:]]/\\\\\\&/g' \
-e 'h' \
-e 's/.*/-include &.gpi.d/' \
-e 'p' \
-e 'g' \
-e 's!.*!$1.d: $$$$(call graphics-source,&)!' \
-e 'p' \
-e 's/.*//' \
-e 'x' \
-e 's!.*!$1.$(build_target_extension) $1._graphics: $$$$(call graphics-target,&)!' \
-e 'p' \
-e 'd' \
$1.log
endef

# Checks for build failure due to pstex inclusion, and gives instructions.
#
# $(call die-on-pstexs,<parsed file>)
define die-on-pstexs
if $(EGREP) -q '^! LaTeX Error: File .*\.pstex.* not found' $1; then \
	$(ECHO) "$(C_ERROR)Missing pstex_t file(s)$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)Please run$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)  make all-pstex$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)before proceeding.$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for the use of import.sty and bails - we don't support subdirectories
#
# $(call die-on-import-sty,<log file>)
define die-on-import-sty
if $(EGREP) -s '/import.sty\)' '$1'; then \
	$(ECHO) "$(C_ERROR)import.sty is not supported - included files must"; \
	$(ECHO) "$(C_ERROR)be in the same directory as the primary document$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for build failure due to dot2tex, and gives instructions.
#
# $(call die-on-dot2tex,<parsed file>)
define die-on-dot2tex
if $(EGREP) -q ' LaTeX Error: File .*\.dot_t.* not found' $1; then \
	$(ECHO) "$(C_ERROR)Missing dot_t file(s)$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)Please run$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)  make all-dot2tex$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)before proceeding.$(C_RESET)"; \
	exit 1; \
fi
endef

# Checks for the existence of a .aux file, and dies with an error message if it
# isn't there.  Note that we pass the file stem in, not the full filename,
# e.g., to check for foo.aux, we call it thus: $(call die-on-no-aux,foo)
#
# $(call die-on-no-aux,<aux stem>)
define die-on-no-aux
if [ ! -e '$1.aux' ]; then \
	$(call colorize-latex-errors,$1.log); \
	$(ECHO) "$(C_ERROR)Error: failed to create $1.aux$(C_RESET)"; \
	exit 1; \
fi
endef

# Outputs all index files to stdout.  Arg 1 is the source file stem, arg 2 is
# the list of targets for the discovered dependency.
#
# $(call get-log-index,<log file stem>,<target files>)
define get-log-index
$(SED) \
-e 's/^No file \(.*\.ind\)\.$$/TARGETS=\1/' \
-e 's/^No file \(.*\.[gn]ls\)\.$$/TARGETS=\1/' \
-e 's/[[:space:]]/\\&/g' \
-e '/^TARGETS=/{' \
-e '  h' \
-e '  s!^TARGETS=!$2: !p' \
-e '  g' \
-e '  s!^TARGETS=\(.*\)!\1: $1.tex!p' \
-e '}' \
-e 'd' \
'$1.log' | $(SORT) | $(UNIQ)
endef


# Outputs all bibliography files to stdout.  Arg 1 is the source stem, arg 2 is
# a list of targets for each dependency found.
#
# The script kills all lines that do not contain bibdata.  Remaining lines have
# the \bibdata macro and delimiters removed to create a dependency list.  A
# trailing comma is added, then all adjacent commas are collapsed into a single
# comma.  Then commas are replaced with the string .bib[space], and the
# trailing space is killed off.  Finally, all filename spaces are escaped.
# This produces a list of space-delimited .bib filenames, which is what the
# make dep file expects to see.
#
# Note that we give kpsewhich a bogus argument so that a failure of sed to
# produce output will not cause an error.
#
# $(call get-bibs,<aux file>,<targets>)
define get-bibs
$(SED) \
-e '/^\\bibdata/!d' \
-e 's/\\bibdata{\([^}]*\)}/\1,/' \
-e 's/,\{2,\}/,/g' \
-e 's/[[:space:]]/\\&/g' \
-e 's/,/.bib /g' \
-e 's/ \{1,\}$$//' \
$1 | $(XARGS) $(KPSEWHICH) '#######' | \
$(SED) \
-e 's!^!$2: !' | \
$(SORT) | $(UNIQ)
endef

# Makes a an aux file that only has stuff relevant to the target in it
# $(call make-auxtarget-file,<flattened-aux>,<new-aux>)
define make-auxtarget-file
$(SED) \
-e '/^\\newlabel/!d' \
$1 > $2
endef

# Makes an aux file that only has stuff relevant to the bbl in it
# $(call make-auxbbl-file,<flattened-aux>,<new-aux>)
define make-auxbbl-file
$(SED) \
-e '/^\\newlabel/d' \
$1 > $2
endef

# Makes a .gpi.d file from a .gpi file
# $(call make-gpi-d,<.gpi>,<.gpi.d>)
define make-gpi-d
$(ECHO) '# vim: ft=make' > $2; \
$(ECHO) 'ifndef INCLUDED_$(call cleanse-filename,$2)' >> $2; \
$(ECHO) 'INCLUDED_$(call cleanse-filename,$2) := 1' >> $2; \
$(call get-gpi-deps,$1,$(addprefix $(2:%.gpi.d=%).,$(GPI_OUTPUT_EXTENSION) gpi.d)) >> $2; \
$(ECHO) 'endif' >> $2;
endef

# Parse .gpi files for data and loaded dependencies, output to stdout
#
# The sed script here tries to be clever about obtaining valid
# filenames from the gpi file.  It assumes that the plot command starts its own
# line, which is not too difficult a constraint to satisfy.
#
# This command script also generates 'include' directives for every 'load'
# command in the .gpi file.  The load command must appear on a line by itself
# and the file it loads must have the suffix .gpi.  If you don't want it to be
# compiled when running make graphics, then give it a suffix of ._include_.gpi.
#
# $(call get-gpi-deps,<gpi file>,<targets>)
define get-gpi-deps
$(SED) \
-e '/^[[:space:]]*s\{0,1\}plot/,/[^\\]$$/{' \
-e ' H' \
-e ' /[^\\]$$/{' \
-e '  s/.*//' \
-e '  x' \
-e '  s/\\\{0,1\}\n//g' \
-e '  s/^[[:space:]]*s\{0,1\}plot[[:space:]]*\(\[[^]]*\][[:space:]]*\)*/,/' \
-e '  s/[[:space:]]*\(['"'"'\'"'"''"'"'"][^'"'"'\'"'"''"'"'"]*['"'"'\'"'"''"'"'"]\)\{0,1\}[^,]*/\1/g' \
-e '  s/,['"'"'\'"'"''"'"'"]-\{0,1\}['"'"'\'"'"''"'"'"]//g' \
-e '  s/[,'"'"'\'"'"''"'"'"]\{1,\}/ /g' \
-e '  s/.*:.*/$$(error Error: Filenames with colons are not allowed: &)/' \
-e '  s!.*!$2: &!' \
-e '  p' \
-e ' }' \
-e ' d' \
-e '}' \
-e 's/^[[:space:]]*load[[:space:]]*['"'"'\'"'"''"'"'"]\([^'"'"'\'"'"''"'"'"]*\.gpi\)['"'"'\'"'"''"'"'"].*$$/-include \1.d/p' \
-e 'd' \
'$1'
endef

# Colorizes real, honest-to-goodness LaTeX errors that can't be overcome with
# recompilation.
#
# Note that we only ignore file not found errors for things that we know how to
# build, like graphics files.
#
# Also note that the output of this is piped through sed again to escape any
# backslashes that might have made it through.  This is to avoid sending things
# like "\right" to echo, which interprets \r as LF.  In bash, we could just do
# ${var//\\/\\\\}, but in other popular sh variants (like dash), this doesn't
# work.
#
# $(call colorize-latex-errors,<log file>)
define colorize-latex-errors
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\(\n\)\(.*\)/\2\1/' \
-e '}' \
-e '/^::P\(P\{1,\}\)::/{' \
-e '  s//::\1::/' \
-e '  G' \
-e '  h' \
-e '  d' \
-e '}' \
-e '/^::P::/{' \
-e '  s//::0::/' \
-e '  G' \
-e '}' \
-e 'b start' \
-e ':needonemore' \
-e 's/^/::P::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needtwomore' \
-e 's/^/::PP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':needthreemore' \
-e 's/^/::PPP::/' \
-e 'G' \
-e 'h' \
-e 'd' \
-e ':start' \
-e '/^! LaTeX Error: File /{' \
-e '  s/\n//g' \
-e '  b needtwomore' \
-e '}' \
-e 's/^[^[:cntrl:]:]*:[[:digit:]]\{1,\}:/!!! &/' \
-e 's/^\(.*\n\)\([^[:cntrl:]:]*:[[:digit:]]\{1,\}: .*\)/\1!!! \2/' \
-e '/^!!! .* LaTeX Error: File /{' \
-e '  s/\n//g' \
-e '  b needonemore' \
-e '}' \
-e '/^::0::! LaTeX Error: File .*/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/^::0::! //' \
-e '  s/^\(.*not found.\).*Enter file name:.*\n\(.*[[:digit:]]\{1,\}\): Emergency stop.*/\2: \1/' \
-e '  b error' \
-e '}' \
-e '/^::0::!!! .*LaTeX Error: File .*/{' \
-e '  /\n\n$$/{' \
-e '    s/^::0:://' \
-e '    b needonemore' \
-e '  }' \
-e '  s/::0::!!! //' \
-e '  /could not locate.*any of these extensions:/{' \
-e '    d' \
-e '  }' \
-e '  s/\(not found\.\).*/\1/' \
-e '  b error' \
-e '}' \
-e '/^\(.* LaTeX Error: Missing .begin.document.\.\).*/{' \
-e '  s//\1 --- Are you trying to build an include file?/' \
-e '  b error' \
-e '}' \
-e '/.*\(!!! .*Undefined control sequence\)[^[:cntrl:]]*\(.*\)/{' \
-e '  s//\1: \2/' \
-e '  s/\nl\.[[:digit:]][^[:cntrl:]]*\(\\[^\\[:cntrl:]]*\).*/\1/' \
-e '  b error' \
-e '}' \
-e '/^\(!pdfTeX error:.*\)s*/{' \
-e '  b error' \
-e '}' \
-e '/.*\(!!! .*\)/{' \
-e '  s//\1/' \
-e '  s/[[:cntrl:]]//' \
-e '  s/[[:cntrl:]]$$//' \
-e '  b error' \
-e '}' \
-e 'd' \
-e ':error' \
-e 's/^!\(!! \)\{0,1\}\(.*\)/$(C_ERROR)\2$(C_RESET)/' \
-e 'p' \
-e 'd' \
'$1' | $(SED) -e 's/\\\\/\\\\\\\\/g'
endef

# Colorize Makeindex errors
define colorize-makeindex-errors
$(SED) \
-e '/^!! /{' \
-e '  N' \
-e '  s/^.*$$/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
'$1'
endef

# Colorize xindy errors
# $(call colorize-xindy-errors,<log file>)
define colorize-xindy-errors
$(SED) \
-e 's/^xindy:.*/$(C_ERROR)&$(C_RESET)/p' \
-e 'd' \
'$1'
endef

# Colorize epstopdf errors
#
# $(call colorize-epstopdf-errors,<log file>)
define colorize-epstopdf-errors
$(SED) \
-e '/^Error:/,/^Execution stack:/{' \
-e '  /^Execution stack:/d' \
-e '  s/.*/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
'$1'
endef

# Colorize GNUplot errors
#
# $(call colorize-gnuplot-errors,<log file>)
define colorize-gnuplot-errors
$(SED) \
-e '/, line [0-9]*:/!{' \
-e '  H' \
-e '  x' \
-e '  s/.*\n\(.*\n.*\)$$/\1/' \
-e '  x' \
-e '}' \
-e '/, line [0-9]*:/{' \
-e '  H' \
-e '  /unknown.*terminal type/{' \
-e '    s/.*/--- Try changing the GNUPLOT_OUTPUT_EXTENSION variable to '"'"'eps'"'"'./' \
-e '    H' \
-e '  }' \
-e '  /gpihead/{' \
-e '    s/.*/--- This could be a Makefile bug - contact the maintainer./' \
-e '    H' \
-e '  }' \
-e '  g' \
-e '  s/.*/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e '/^gnuplot>/,/^$$/{' \
-e '  s/^gnuplot.*/$(C_ERROR)&/' \
-e '  s/^$$/$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
$1
endef

# Colorize GraphViz errors
#
# $(call colorize-dot-errors,<log file>)
define colorize-dot-errors
$(SED) \
-e 's/.*not found.*/$(C_ERROR)&$(C_RESET)/p' \
-e '/^Error:/,/context:/s/.*/$(C_ERROR)&$(C_RESET)/p' \
-e 's/^Warning:.*/$(C_WARNING)&$(C_RESET)/p' \
-e 'd' \
'$1'
endef

# Get all important .aux files from the top-level .aux file and merges them all
# into a single file, which it outputs to stdout.
#
# $(call flatten-aux,<toplevel aux>,<output file>)
define flatten-aux
$(SED) \
-e '/\\@input{\(.*\)}/{' \
-e     's//\1/' \
-e     's![.:]!\\&!g' \
-e     'h' \
-e     's!.*!\\:\\\\@input{&}:{!' \
-e     'p' \
-e     'x' \
-e     's/\\././g' \
-e     's/.*/r &/p' \
-e     's/.*/d/p' \
-e     's/.*/}/p' \
-e     'd' \
-e '}' \
-e 'd' \
'$1' > "$1.$$$$.sed.make"; \
$(SED) -f "$1.$$$$.sed.make" '$1' > "$1.$$$$.make"; \
$(SED) \
-e '/^\\relax/d' \
-e '/^\\bibcite/d' \
-e 's/^\(\\newlabel{[^}]\{1,\}}\).*/\1/' \
"$1.$$$$.make" | $(SORT) > '$2'; \
$(call remove-temporary-files,$1.$$$$.make $1.$$$$.sed.make)
endef

# Generate pdf from postscript
#
# Note that we don't just call ps2pdf, since there are so many versions of that
# script on various systems.  Instead, we call the postscript interpreter
# directly.
#
# $(call ps2pdf,infile,outfile,[embed fonts])
define ps2pdf
	$(GS) \
		-dSAFER -dCompatibilityLevel=$(PS_COMPATIBILITY) \
		$(if $3,$(PS_EMBED_OPTIONS)) \
		-q -dNOPAUSE -dBATCH \
		-sDEVICE=pdfwrite -sstdout=%stderr \
		'-sOutputFile=$2' \
		-dSAFER -dCompatibilityLevel=$(PS_COMPATIBILITY) \
		$(if $3,$(PS_EMBED_OPTIONS)) \
		-c .setpdfwrite \
		-f '$1'
endef

# Colorize LaTeX output.
color_tex := \
$(SED) \
-e '$${' \
-e '  /^$$/!{' \
-e '    H' \
-e '    s/.*//' \
-e '  }' \
-e '}' \
-e '/^$$/!{' \
-e '  H' \
-e '  d' \
-e '}' \
-e '/^$$/{' \
-e '  x' \
-e '  s/^\n//' \
-e '  /Output written on /{' \
-e '    s/.*Output written on \([^(]*\) (\([^)]\{1,\}\)).*/Success!  Wrote \2 to \1/' \
-e '    s/[[:digit:]]\{1,\}/$(C_PAGES)&$(C_RESET)/g' \
-e '    s/Success!/$(C_SUCCESS)&$(C_RESET)/g' \
-e '    s/to \(.*\)$$/to $(C_SUCCESS)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  / *LaTeX Error:.*/{' \
-e '    s/.*\( *LaTeX Error:.*\)/$(C_ERROR)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /.*Warning:.*/{' \
-e '    s//$(C_WARNING)&$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /Underfull.*/{' \
-e '    s/.*\(Underfull.*\)/$(C_UNDERFULL)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  /Overfull.*/{' \
-e '    s/.*\(Overfull.*\)/$(C_OVERFULL)\1$(C_RESET)/' \
-e '    b end' \
-e '  }' \
-e '  d' \
-e '  :end' \
-e '  G' \
-e '}'

# Colorize BibTeX output.
color_bib := \
$(SED) \
-e 's/^Warning--.*/$(C_WARNING)&$(C_RESET)/' \
-e 't' \
-e '/---/,/^.[^:]/{' \
-e '  H' \
-e '  /^.[^:]/{' \
-e '    x' \
-e '    s/\n\(.*\)/$(C_ERROR)\1$(C_RESET)/' \
-e '    p' \
-e '    s/.*//' \
-e '    h' \
-e '    d' \
-e '  }' \
-e '  d' \
-e '}' \
-e '/(.*error.*)/s//$(C_ERROR)&$(C_RESET)/' \
-e 'd'

# Make beamer output big enough to print on a full page.  Landscape doesn't
# seem to work correctly.
enlarge_beamer	= $(PSNUP) -l -1 -W128mm -H96mm -pletter

# $(call test-run-again,<source stem>)
test-run-again	= $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.)$$' $1.log

# This tests whether the build target commands should be run at all, from
# viewing the log file.
# $(call test-log-for-need-to-run,<source stem>)
define test-log-for-need-to-run
$(SED) \
-e '/^No file $(call escape-fname-regex,$1)\.aux\./d' \
$1.log \
| $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.|No file .+\.tex\.|LaTeX Warning: File.*)$$'
endef

# LaTeX invocations
#
# $(call latex,<tex file>,[<extra LaTeX args>])
run-latex	= $(latex_build_program) -interaction=batchmode -file-line-error $(if $2,$2,) $1 > /dev/null

# $(call latex-color-log,<LaTeX stem>)
latex-color-log	= $(color_tex) $1.log

# $(call run-makeindex,<input>,<output>,<log>,[.ist style file])
define run-makeindex
success=1; \
if ! $(MAKEINDEX) -q $1 -t $3 -o $2 $(if $4,-s $4,) > /dev/null || $(EGREP) -q '^!!' $3; \
then \
	$(call colorize-makeindex-errors,$3); \
	$(RM) -f '$2'; \
	success=0; \
fi; \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef


# $(call run-xindy,<input>,<output>,<module>,<log>)
define run-xindy
success=1; \
if ! $(XINDY) -q -o $2 -L $(XINDYLANG) -C $(XINDYENC) -I xindy -M $3 -t $4 $1 > /dev/null || $(EGREP) -q '^xindy:' $4; then \
	$(call colorize-xindy-errors,$4); \
	$(RM) -f '$2'; \
	success=0; \
fi; \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# This runs the given script to generate output, and it uses MAKE_RESTARTS to
# ensure that it never runs it more than once for a particular root make
# invocation.
#
# $(call run-script,<interpreter>,<input>,<output>)
define run-script
[ ! -e '$2.cookie' ] && $(ECHO) "restarts=$(RESTARTS)" > $2.cookie && $(ECHO) "level=$(MAKELEVEL)" >> $2.cookie; \
restarts=`$(SED) -n -e 's/^restarts=//p' $2.cookie`; \
level=`$(SED) -n -e 's/^level=//p' $2.cookie`; \
if $(EXPR) $(MAKELEVEL) '<=' $$level '&' $(RESTARTS) '<=' $$restarts >/dev/null; then \
	$(call echo-build,$2,$3,$(RESTARTS)-$(MAKELEVEL)); \
	$1 '$2' '$3'; \
	$(ECHO) "restarts=$(RESTARTS)" > '$2.cookie'; \
	$(ECHO) "level=$(MAKELEVEL)" >> '$2.cookie'; \
fi
endef

# BibTeX invocations
#
# $(call run-bibtex,<tex stem>)
run-bibtex	= $(BIBTEX) $1 | $(color_bib)


# $(call convert-eps-to-pdf,<eps file>,<pdf file>,[gray])
# Note that we don't use the --filter flag because it has trouble with bounding boxes that way.
define convert-eps-to-pdf
$(if $3,$(CAT) '$1' | $(call kill-ps-color) > '$1.cookie',$(CP) '$1' '$1.cookie'); \
$(EPSTOPDF) '$1.cookie' --outfile='$2' > $1.log; \
$(call colorize-epstopdf-errors,$1.log);
endef

# $(call default-gpi-fontsize,<output file>)
#
# Find the default fontsize given the *output* file (it is based on the output extension)
#
default-gpi-fontsize = $(if $(filter %.pdf,$1),$(DEFAULT_GPI_PDF_FONTSIZE),$(DEFAULT_GPI_EPS_FONTSIZE))

# $(call gpi-fontsize,<gpi file>,<output file>)
#
# Find out what the gnuplot fontsize should be.  Tries, in this order:
# - ##FONTSIZE comment in gpi file
# - ##FONTSIZE comment in global gpi file
# - default fontsize based on output type
define gpi-fontsize
$(strip $(firstword \
	$(shell $(SED) -e 's/^\#\#FONTSIZE=\([[:digit:]]\{1,\}\)/\1/p' -e 'd' $1 $(strip $(gpi_global))) \
	$(call default-gpi-fontsize,$2)))
endef

# $(call gpi-monochrome,<gpi file>,[gray])
define gpi-monochrome
$(strip $(if $2,monochrome,$(if $(shell $(EGREP) '^\#\#[[:space:]]*GRAY[[:space:]]*$$' $1 $(gpi_global)),monochrome,color)))
endef

# $(call gpi-font-entry,<output file>,<fontsize>)
#
# Get the font entry given the output file (type) and the font size.  For PDF
# it uses fsize or font, for eps it just uses the bare number.
gpi-font-entry = $(if $(filter %.pdf,$1),$(subst FONTSIZE,$2,$(GPI_FSIZE_SYNTAX)),$2)

# $(call gpi-terminal,<gpi file><output file>,[gray])
#
# Get the terminal settings for a given gpi and its intended output file
define gpi-terminal
$(if $(filter %.pdf,$2),pdf enhanced,postscript enhanced eps) \
$(call gpi-font-entry,$2,$(call gpi-fontsize,$1,$2)) \
$(call gpi-monochrome,$1,$3)
endef

# $(call gpi-embed-pdf-fonts,<input file>,<output file>)
#
define gpi-embed-pdf-fonts
$(GS) \
	-q \
	-dSAFER \
	-dNOPAUSE \
	-dBATCH \
	-sDEVICE=$(if $(filter pdf,$(GPI_OUTPUT_EXTENSION)),pdfwrite,pswrite) \
	-sOutputFile='$2' \
	-sstdout=%stderr \
	-dCompatibilityLevel=1.5 \
	-dPDFSETTINGS=/prepress \
	-c .setpdfwrite \
	-f '$1'
endef

# $(call convert-gpi,<gpi file>,<output file>,[gray])
#
define convert-gpi
$(ECHO) 'set terminal $(call gpi-terminal,$1,$2,$3)' > $1head.make; \
$(ECHO) 'set output "$2"' >> $1head.make; \
$(if $(gpi_global),$(CAT) $(gpi_global) >> $1head.make;,) \
fnames='$1head.make $1';\
$(if $(gpi_sed),\
	$(SED) -f '$(gpi_sed)' $$fnames > $1.temp.make; \
	fnames=$1.temp.make;,\
) \
success=1; \
if ! $(GNUPLOT) $$fnames 2>$1.log; then \
	$(call colorize-gnuplot-errors,$1.log); \
	success=0; \
else \
	if ! $(call gpi-embed-pdf-fonts,$2,$2.embed.make); then \
		success = 0; \
	else \
		$(call move-if-exists,$2.embed.make,$2); \
	fi; \
fi; \
$(if $(gpi_sed),$(call remove-temporary-files,$1.temp.make);,) \
$(call remove-temporary-files,$1head.make); \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# Creation of .eps files from .png files
#
# The intermediate step of PNM (using NetPBM) produces much nicer output than
# ImageMagick's "convert" binary.  I couldn't get the right combination of
# flags to make it look nice, anyway.
#
# To handle gray scale conversion, we pipe things through ppmtopgm in the
# middle.
#
# $(call convert-png,<png file>,<eps file>)
define convert-png
$(PNGTOPNM) "$1" \
	$(if $3,| $(PPMTOPGM),) \
	| $(PNMTOPS) -noturn \
	> "$2"
endef

# Creation of .eps files from .jpg/.jpeg files
#
# Thanks to brubakee for this solution.
#
# Uses Postscript level 2 to avoid file size bloat
# $(call convert-jpg,<jpg file>,<eps file>)
define convert-jpg
$(CONVERT) $(if $3,-type Grayscale,) '$1' eps2:'$2'
endef

# Creation of .eps files from .fig files
# $(call convert-fig,<fig file>,<output file>,[gray])
convert-fig	= $(FIG2DEV) -L $(if $(filter %.pdf,$2),pdf,eps) $(if $3,-N,) $1 $2

# Creation of .pstex files from .fig files
# $(call convert-fig-pstex,<fig file>,<pstex file>)
convert-fig-pstex	= $(FIG2DEV) -L pstex $1 $2 > /dev/null 2>&1

# Creation of .pstex_t files from .fig files
# $(call convert-fig-pstex-t,<fig file>,<pstex file>,<pstex_t file>)
convert-fig-pstex-t	= $(FIG2DEV) -L pstex_t -p $3 $1 $2 > /dev/null 2>&1

# Creation of .dot_t files from .dot files
# #(call convert-dot-tex,<dot file>,<dot_t file>)
convert-dot-tex		= $(DOT2TEX) '$1' > '$2'

# Converts svg files into .eps files
#
# $(call convert-svg,<svg file>,<eps/pdf file>,[gray])
convert-svg	= $(INKSCAPE) --without-gui $(if $(filter %.pdf,$2),--export-pdf,--export-eps)='$2' '$1'

# Converts xvg files into .eps files
#
# $(call convert-xvg,<xvg file>,<eps file>,[gray])
convert-xvg	= $(XMGRACE) '$1' -printfile - -hardcopy -hdevice $(if $3,-mono,) EPS > '$2'

# Converts .eps.gz files into .eps files
#
# $(call convert-epsgz,<eps.gz file>,<eps file>,[gray])
convert-epsgz	= $(GUNZIP) -c '$1' $(if $3,| $(call kill-ps-color)) > '$2'

# Converts .eps files into .eps files (usually a no-op, but can make grayscale)
#
# $(call convert-eps,<in file>,<out file>,[gray])
convert-eps	= $(if $3,$(call kill-ps-color) $1 > $2)

# The name of the file containing special postscript commands for grayscale
gray_eps_file	:= gray.eps.make

# Changes sethsbcolor and setrgbcolor calls in postscript to always produce
# grayscale.  In general, this is accomplished by writing new versions of those
# functions into the user dictionary space, which is looked up before the
# global or system dictionaries (userdict is one of the permanent dictionaries
# in postscript and is not read-only like systemdict).
#
# For setrgbcolor, the weighted average of the triple is computed and the
# triple is replaced with three copies of that average before the original
# procedure is called: .299R + .587G + .114B
#
# For sethsbcolor, the color is first converted to RGB, then to grayscale by
# the new setrgbcolor operator as described above.  Why is this done?
# Because simply using the value component will tend to make pure colors
# white, a very undesirable thing.  Pure blue should not translate to white,
# but to some level of gray.  Conversion to RGB does the right thing.  It's
# messy, but it works.
#
# From
# http://en.wikipedia.org/wiki/HSV_color_space#Transformation_from_HSV_to_RGB,
# HSB = HSV (Value = Brightness), and the formula used to convert to RGB is
# as follows:
#
# Hi = int(floor(6 * H)) mod 6
# f = 6 * H - Hi
# p = V(1-S)
# q = V(1-fS)
# t = V(1-(1-f)S)
# if Hi = 0: R G B <-- V t p
# if Hi = 1: R G B <-- q V p
# if Hi = 2: R G B <-- p V t
# if Hi = 3: R G B <-- p q V
# if Hi = 4: R G B <-- t p V
# if Hi = 5: R G B <-- V p q
#
# The messy stack-based implementation is below
# $(call create-gray-eps-file,filename)
define create-gray-eps-file
$(ECHO) -n -e '\
/OLDRGB /setrgbcolor load def\n\
/setrgbcolor {\n\
    .114 mul exch\n\
    .587 mul add exch\n\
    .299 mul add\n\
    dup dup\n\
    OLDRGB\n\
} bind def\n\
/OLDHSB /sethsbcolor load def\n\
/sethsbcolor {\n\
    2 index                     % H V S H\n\
    6 mul floor cvi 6 mod       % Hi V S H\n\
    3 index                     % H Hi V S H\n\
    6 mul                       % 6H Hi V S H\n\
    1 index                     % Hi 6H Hi V S H\n\
    sub                         % f Hi V S H\n\
    2 index 1                   % 1 V f Hi V S H\n\
    4 index                     % S 1 V f Hi V S H\n\
    sub mul                     % p f Hi V S H\n\
    3 index 1                   % 1 V p f Hi V S H\n\
    6 index                     % S 1 V p f Hi V S H\n\
    4 index                     % f S 1 V p f Hi V S H\n\
    mul sub mul                 % q p f Hi V S H\n\
    4 index 1 1                 % 1 1 V q p f Hi V S H\n\
    5 index                     % f 1 1 V q p f Hi V S H\n\
    sub                         % (1-f) 1 V q p f Hi V S H\n\
    8 index                     % S (1-f) 1 V q p f Hi V S H\n\
    mul sub mul                 % t q p f Hi V S H\n\
    4 -1 roll pop               % t q p Hi V S H\n\
    7 -2 roll pop pop           % t q p Hi V\n\
    5 -2 roll                   % Hi V t q p\n\
    dup 0 eq\n\
    {1 index 3 index 6 index}\n\
    {\n\
        dup 1 eq\n\
        {3 index 2 index 6 index}\n\
        {\n\
            dup 2 eq\n\
            {4 index 2 index 4 index}\n\
            {\n\
                dup 3 eq\n\
                {4 index 4 index 3 index}\n\
                {\n\
                    dup 4 eq\n\
                    {2 index 5 index 3 index}\n\
                    {\n\
                        dup 5 eq\n\
                        {1 index 5 index 5 index}\n\
                        {0 0 0}\n\
                        ifelse\n\
                    }\n\
                    ifelse\n\
                }\n\
                ifelse\n\
            }\n\
            ifelse\n\
        }\n\
        ifelse\n\
    }\n\
    ifelse                      % B G R Hi V t q p\n\
    setrgbcolor\n\
    5 {pop} repeat\n\
} bind def\n'\
> $1
endef

# This actually inserts the color-killing code into a postscript file
# $(call kill-ps-color)
define kill-ps-color
$(SED) -e '/%%EndComments/r $(gray_eps_file)'
endef

# Converts graphviz .dot files into .eps files
# Grayscale is not directly supported by dot, so we pipe it through fig2dev in
# that case.
# $(call convert-dot,<dot file>,<eps file>,<log file>,[gray])
define convert-dot
$(DOT) -Tps '$1' 2>'$3' $(if $4,| $(call kill-ps-color)) > $2; \
$(call colorize-dot-errors,$3)
endef

# Convert DVI to Postscript
# $(call make-ps,<dvi file>,<ps file>,<log file>,[<paper size>])
make-ps		= \
	$(DVIPS) -z -o '$2' $(if $(filter-out BEAMER,$4),-t$(firstword $4),) '$1' \
		$(if $(filter BEAMER,$4),| $(enlarge_beamer)) > $3 2>&1

# Convert Postscript to PDF
# $(call make-pdf,<ps file>,<pdf file>,<log file>,<embed file>)
make-pdf	= \
	$(call ps2pdf,$1,$2,$(filter 1,$(shell $(CAT) '$4'))) > '$3' 2>&1

# Display information about what is being done
# $(call echo-build,<input file>,<output file>,[<run number>])
echo-build	= $(ECHO) "$(C_BUILD)= $1 --> $2$(if $3, ($3),) =$(C_RESET)"
echo-graphic	= $(ECHO) "$(C_GRAPHIC)= $1 --> $2 =$(C_RESET)"
echo-dep	= $(ECHO) "$(C_DEP)= $1 --> $2 =$(C_RESET)"

# Display a list of something
# $(call echo-list,<values>)
echo-list	= for x in $1; do $(ECHO) "$$x"; done

#
# DEFAULT TARGET
#

.PHONY: all
all: $(default_pdf_targets) ;

.PHONY: all-pdf
all-pdf: $(default_pdf_targets) ;

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.PHONY: all-ps
all-ps: $(default_ps_targets) ;

.PHONY: all-dvi
all-dvi: $(default_dvi_targets) ;
endif

#
# VIEWING TARGET
#
.PHONY: show
show: all
	$(QUIET)for x in $(default_pdf_targets); do \
		[ -e "$$x" ] && $(VIEW_PDF) $$x & \
	done

#
# INCLUDES
#
source_includes	:= $(addsuffix .d,$(source_stems_to_include))
graphic_includes := $(addsuffix .gpi.d,$(graphic_stems_to_include))

# Check the version of the makefile
ifneq "" "$(filter 3.79 3.80,$(MAKE_VERSION))"
$(warning $(C_WARNING)Your version of make is too old.  Please upgrade.$(C_RESET))
endif

# Include only the dependencies used
ifneq "" "$(source_includes)"
include $(source_includes)$(call include-message,$(source_includes))
endif
ifneq "" "$(graphic_includes)"
include $(graphic_includes)$(call include-message,$(graphic_includes))
endif

#
# MAIN TARGETS
#

# Note that we don't just say %: %.pdf here - this can tend to mess up our
# includes, which detect what kind of file we are asking for.  For example,
# asking to build foo.pdf is much different than asking to build foo when
# foo.gpi exists, because we look through all of the goals for *.pdf that
# matches *.gpi, then use that to determine which include files we need to
# build.
#
# Thus, we invoke make recursively with better arugments instead, restarting
# all of the appropriate machinery.
.PHONY: $(default_stems_ss)
$(default_stems_ss): %: %.pdf ;

# This builds and displays the wanted file.
.PHONY: $(addsuffix ._show,$(stems_ssg))
$(addsuffix ._show,$(stems_ssg)): %._show: %.pdf
	$(QUIET)$(VIEW_PDF) $< &

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.SECONDARY: $(all_pdf_targets)
%.pdf: %.ps %.embed.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-pdf,$<,$@.temp,$@.log,$*.embed.make); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(RM) -f '$@'; \
	    $(MV) '$@.temp' '$@'; \
	    $(TOUCH) '$@'; \
	    $(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi

.SECONDARY: $(all_ps_targets)
%.ps: %.dvi %.paper.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-ps,$<,$@.temp,$@.log,\
			$(firstword $(shell $(CAT) $*.paper.make))); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(RM) -f '$@'; \
	    $(MV) '$@.temp' '$@'; \
	    $(TOUCH) '$@'; \
	    $(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi
endif

# Build the final target (dvi or pdf) file.  This is a very tricky rule because
# of the way that latex runs multiple times, needs graphics after the first run
# (or maybe already has them), and relies on bibliographies or indices that may
# not exist.
#
#	Check the log for fatal errors.  If they exist, colorize and bail.
#
#	Create the .auxtarget.cookie file.  (Needed for next time if not present)
#
#	If any of the following are true, we must rebuild at least one time:
#
#	* the .bbl was recently rebuilt
#
#		check a cookie, then delete it
#
#	* any of several output files was created or changed:
#
#		check $*.run.cookie, then delete it
#
#	* the .aux file changed in a way that necessitates attention
#
#		Note that if the .auxtarget.make file doesn't exist, this means
#		that we are doing a clean build, so it doesn't figure into the
#		test for running again.
#
#		compare against .auxtarget.make
#
#		move if different, remove if not
#
#	* the .log file has errors or warnings requiring at least one more run
#
#	We use a loop over a single item to simplify the process of breaking
#	out when we find one of the conditions to be true.
#
#	If we do NOT need to run latex here, then we move the $@.1st.make file
#	over to $@ because the target file has already been built by the first
#	dependency run and is valid.
#
#	If we do, we delete that cookie file and do the normal multiple-runs
#	routine.
#
ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.SECONDARY: $(all_dvi_targets)
endif
%.$(build_target_extension): %.bbl %.aux %.$(build_target_extension).1st.make
	$(QUIET)\
	fatal=`$(call colorize-latex-errors,$*.log)`; \
	if [ x"$$fatal" != x"" ]; then \
		$(ECHO) "$$fatal"; \
		exit 1; \
	fi; \
	$(call make-auxtarget-file,$*.aux.make,$*.auxtarget.cookie); \
	run=0; \
	for i in 1; do \
		if $(call test-exists,$*.bbl.cookie); then \
			run=1; \
			break; \
		fi; \
		if $(call test-exists,$*.run.cookie); then \
			run=1; \
		    	break; \
		fi; \
		if $(call \
		test-exists-and-different,$*.auxtarget.cookie,$*.auxtarget.make);\
		then \
			run=1; \
			break; \
		fi; \
		if $(call test-log-for-need-to-run,$*); then \
			run=1; \
			break; \
		fi; \
		if [ ! -e $*.1st.*.make ]; then \
			run=1; \
			break; \
		fi; \
	done; \
	$(call remove-temporary-files,$*.bbl.cookie $*.run.cookie); \
	$(MV) $*.auxtarget.cookie $*.auxtarget.make; \
	if [ x"$$run" = x"1" ]; then \
		$(call remove-files,$@.1st.make); \
		for i in 2 3 4 5; do \
			$(if $(findstring 3.79,$(MAKE_VERSION)),\
				$(call echo-build,$*.tex,$@,$(RESTARTS)-$$$$i),\
				$(call echo-build,$*.tex,$@,$(RESTARTS)-$$i)\
			); \
			$(call run-latex,$*); \
			$(CP) '$*.log' '$*.'$(RESTARTS)-$$i'.log'; \
			$(call test-run-again,$*) || break; \
		done; \
	else \
		$(MV) '$@.1st.make' '$@'; \
	fi; \
	$(call copy-with-logging,$@,$(BINARY_TARGET_DIR)); \
	$(call latex-color-log,$*)

# Build the .bbl file.  When dependencies are included, this will (or will
# not!) depend on something.bib, which we detect, acting accordingly.  The
# dependency creation also produces the %.auxbbl.make file.  BibTeX is a bit
# finicky about what you call the actual files, but we can rest assured that if
# a .auxbbl.make file exists, then the .aux file does, as well.  The
# .auxbbl.make file is a cookie indicating whether the .bbl needs to be
# rewritten.  It only changes if the .aux file changes in ways relevant to .bbl
# creation.
#
# Note that we do NOT touch the .bbl file if there is no need to
# create/recreate it.  We would like to leave existing files alone if they
# don't need to be changed, thus possibly avoiding a rebuild trigger.
%.bbl: %.auxbbl.make
	$(QUIET)\
	$(if $(filter %.bib,$^),\
		$(call echo-build,$(filter %.bib,$?) $*.aux,$@); \
		$(call run-bibtex,$*); \
		$(TOUCH) $@.cookie; \
	) \
	if $(EGREP) -q 'bibstyle.(apacite|apacann|chcagoa|[^}]*annot)' '$*.aux'; then \
		$(call echo-build,** annotated extra latex **,output ignored,$(RESTARTS)-1); \
		$(call run-latex,$*); \
		$(CP) '$*.log' '$*.$(RESTARTS)-annotated.log'; \
		$(if $(filter %.bib,$^),\
			$(call echo-build,** annotated extra bibtex ** $(filter %.bib,$?) $*.aux,$@); \
			$(call run-bibtex,$*); \
			$(TOUCH) $@.cookie; \
		) \
		$(call echo-build,** annotated extra latex **,output ignored,$(RESTARTS)-2); \
		$(call run-latex,$*); \
	fi

# Create the index file - note that we do *not* depend on %.tex here, since
# that unnecessarily restricts the kinds of indices that we can build to those
# with exactly the same stem as the source file.  Things like splitidx create
# idx files with other names.
#
# Therefore, we add the .tex dependency in the sourcestem.d file in the call to
# get index file dependencies from the logs.
%.ind:	%.idx
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.ilg)

# Create a glossary file from a .ist file
%.gls:	%.glo %.tex %.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.glg,$*.ist)

# Create a glossary file from a glossary input formatted for xindy
%.gls:	%.glo %.tex %.xdy
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-xindy,$<,$@,$*,$*.glg)

# Create the glossary file from a nomenclature file
%.gls:	%.glo %.tex nomencl.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.glg,nomencl.ist)

# Create the nomenclature file
%.nls:	%.nlo %.tex nomencl.ist
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$<,$@,$*.nlg,nomencl.ist)

# SCRIPTED LaTeX TARGETS
#
# Keep the generated .tex files around for debugging if needed.
.SECONDARY: $(all_tex_targets)

%.tex::	%.tex.sh
	$(QUIET)$(call run-script,$(SHELL),$<,$@)

%.tex::	%.tex.py
	$(QUIET)$(call run-script,$(PYTHON),$<,$@)

%.tex::	%.tex.pl
	$(QUIET)$(call run-script,$(PERL),$<,$@)

%.tex::	%.rst $(RST_STYLE_FILE)
	$(QUIET)\
	$(call run-script,$(RST2LATEX)\
		--documentoptions=letterpaper\
		$(if $(RST_STYLE_FILE),--stylesheet=$(RST_STYLE_FILE),),$<,$@)

#
# GRAPHICS TARGETS
#
.PHONY: all-graphics
all-graphics:	$(all_graphics_targets);

ifeq "$(strip $(BUILD_STRATEGY))" "latex"
.PHONY: all-pstex
all-pstex:	$(all_pstex_targets);
endif

.PHONY: all-dot2tex
all-dot2tex:	$(all_dot2tex_targets);

.PHONY: show-graphics
show-graphics: all-graphics
	$(VIEW_GRAPHICS) $(all_known_graphics)

$(gray_eps_file):
	$(QUIET)$(call echo-build,$^,$@)
	$(QUIET)$(call create-gray-eps-file,$@)

ifeq "$(strip $(BUILD_STRATEGY))" "pdflatex"
%.pdf: %.eps $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-eps-to-pdf,$<,$@,$(GRAY))

ifeq "$(strip $(GPI_OUTPUT_EXTENSION))" "pdf"
%.pdf:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))
endif

%.pdf:	%.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

%.pdf:	%.svg
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-svg,$<,$@,$(GRAY))
endif

ifeq "$(strip $(BUILD_STRATEGY))" "xelatex"
%.pdf: %.eps $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-eps-to-pdf,$<,$@,$(GRAY))

ifeq "$(strip $(GPI_OUTPUT_EXTENSION))" "pdf"
%.pdf:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))
endif

%.pdf:	%.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

endif


%.eps:	%.gpi %.gpi.d $(gpi_sed) $(gpi_global)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))

%.eps: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

%.eps: %.dot $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot,$<,$@,$<.log,$(GRAY))

%.eps: %.xvg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-xvg,$<,$@,$(GRAY))

ifneq "$(default_graphic_extension)" "pdf"
# We have a perfectly good build rule for svg to pdf, so we eliminate this to
# avoid confusing make (it sometimes chooses to go svg -> eps -> pdf).
%.eps: %.svg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-svg,$<,$@,$(GRAY))

# Similarly for these, we don't need eps if we have supported extensions
# already.
%.eps: %.jpg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-jpg,$<,$@,$(GRAY))

%.eps: %.jpeg $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-jpg,$<,$@,$(GRAY))

%.eps: %.png $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-png,$<,$@,$(GRAY))
endif

%.eps: %.eps.gz $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-epsgz,$<,$@,$(GRAY))

%.pstex: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex,$<,$@,$(GRAY))

%.pstex_t: %.fig %.pstex
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex-t,$<,$@,$*.pstex,$(GRAY))

%.dot_t: %.dot
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot-tex,$<,$@)

#
# DEPENDENCY-RELATED TARGETS.
#

# Generate all of the information needed to get dependencies
# As a side effect, this creates a .dvi or .pdf file (depending on the build
# strategy).  We need to be sure to remove it if there are errors.  Errors can
# take several forms and all of them are found within the log file:
#	* There was a LaTeX error
#	* A needed file was not found
#	* Cross references need adjustment
#
# Behavior:
#	This rule is responsible for generating the following:
#	%.aux
#	%.d
#	%.aux.make
#	%.(pdf|dvi).1st.make (the .pdf or .dvi output file, moved)
#
#	Steps:
#
#	Run latex
#	Move .pdf or .dvi somewhere else (make no judgements about success)
#	Flatten the .aux file into another file
#	Add source dependencies
#	Add graphic dependencies
#	Add bib dependencies
#
#	Create cookies for various suffixes that may represent files that
#	need to be read by LaTeX in order for it to function properly.
#
#	Note that if some of the dependencies are discovered because they turn
#	up missing in the log file, we really need the .d file to be reloaded.
#	Adding a sleep command helps with this.  Otherwise make is extremely
#	nondeterministic, sometimes working, sometimes not.
#
#	Usually we can force this by simply removing the generated pdf file and
#	not creating a .1st.make file..
#
%.$(build_target_extension).1st.make %.d %.aux %.aux.make %.fls: %.tex
	$(QUIET)$(call echo-build,$<,$*.d $*.$(build_target_extension).1st.make,$(RESTARTS)-1)
	$(QUIET)\
	$(call run-latex,$<,-recorder) || $(sh_true); \
	$(CP) '$*.log' '$*.$(RESTARTS)-1.log'; \
	$(call die-on-import-sty,$*.log); \
	$(call die-on-dot2tex,$*.log); \
	$(call die-on-no-aux,$*); \
	$(call flatten-aux,$*.aux,$*.aux.make); \
	$(ECHO) "# vim: ft=make" > $*.d; \
	$(ECHO) ".PHONY: $*._graphics" >> $*.d; \
	$(call get-inputs,$*.fls,$(addprefix $*.,aux aux.make d $(build_target_extension))) >> $*.d; \
	$(call get-missing-inputs,$*.log,$(addprefix $*.,aux aux.make d $(build_target_extension))) >> $*.d; \
	$(ECHO) ".SECONDEXPANSION:" >> $*.d; \
	$(call get-graphics,$*) >> $*.d; \
	$(call get-log-index,$*,$(addprefix $*.,aux aux.make)) >> $*.d; \
	$(call get-bibs,$*.aux.make,$(addprefix $*.,bbl aux aux.make)) >> $*.d; \
	$(EGREP) -q "# MISSING" $*.d && $(SLEEP) 1 && $(RM) $*.pdf; \
	$(call move-if-exists,$*.$(build_target_extension),$*.$(build_target_extension).1st.make); \
	for s in toc out lot lof lol nav; do \
		if [ -e "$*.$$s" ]; then \
			if ! $(DIFF) -q $*.$$s $*.$$s.make >/dev/null 2>&1; then \
				$(TOUCH) $*.run.cookie; \
			fi; \
			$(CP) $*.$$s $*.$$s.make; \
		fi; \
	done

# This is a cookie that is updated if the flattened aux file has changed in a
# way that affects the bibliography generation.
.SECONDARY: $(addsuffix .auxbbl.make,$(stems_ssg))
%.auxbbl.make: %.aux.make
	$(QUIET)\
	$(call make-auxbbl-file,$<,$@.temp); \
	$(call replace-if-different-and-remove,$@.temp,$@)

# Build a dependency file for .gpi files.  These often plot data files that
# also reside in the directory, so if a data file changes, it's nice to know
# about it.  This also handles loaded .gpi files, whose filename should have
# _include_. in it.
%.gpi.d: %.gpi
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-gpi-d,$<,$@)

# Store the paper size for this document -- note that if beamer is used we set
# it to the special BEAMER paper size.  We only do this, however, if the
# special comment exists, in which case we enlarge the output with psnup.
#
#	The paper size is extracted from a documentclass attribute.
%.paper.make: %.tex
	$(QUIET)$(SED) \
	-e '/\\documentclass/,/}/{' \
	-e '  s/%.*//' \
	-e '  H' \
	-e '  /}/{' \
	-e '    s/.*//' \
	-e '    x' \
	-e '    /\\documentclass/!d' \
	-e '    s/[\n[:space:]]*//g' \
	-e '    s/\([,{[]\)\([[:alnum:]]\{1,\}\)paper\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/\([,{[]\)\(landscape\)\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/^[^%]*%-//' \
	-e '    s/-%[^%]*$$//' \
	-e '    s/-%[^%]%-/ /g' \
	-e '    p' \
	-e '  }' \
	-e '  d' \
	-e '}' \
	-e 'd' \
	$< > $@; \
	$(EGREP) -q '^[^%]*\\documentclass[^{]*{beamer}' $< && \
	(\
		$(EGREP) -q '^%%[[:space:]]*BEAMER[[:space:]]*LARGE$$' $< && \
		$(ECHO) "BEAMER" > $@ || \
		: > $@ \
	) || $(sh_true)

# Store embedding instructions for this document using a special comment
%.embed.make: %.tex
	$(QUIET)$(EGREP) '^%%[[:space:]]*NO[[:space:]]*EMBED[[:space:]]*$$' $< \
		&& $(ECHO) '' > $@ \
		|| $(ECHO) '1' > $@;

#
# HELPFUL PHONY TARGETS
#

.PHONY: _all_programs
_all_programs:
	$(QUIET)$(ECHO) "== All External Programs Used =="
	$(QUIET)$(call output-all-programs)

.PHONY: _check_programs
_check_programs:
	$(QUIET)$(ECHO) "== Checking Makefile Dependencies =="; $(ECHO)
	$(QUIET) \
	allprogs=`\
	 ($(call output-all-programs)) | \
	 $(SED) \
	 -e 's/^[[:space:]]*//' \
	 -e '/^#/d' \
	 -e 's/[[:space:]]*#.*//' \
	 -e '/^=/s/[[:space:]]/_/g' \
	 -e '/^[[:space:]]*$$/d' \
	 -e 's/^[^=].*=[[:space:]]*\([^[:space:]]\{1,\}\).*$$/\\1/' \
	 `; \
	spaces='                             '; \
	for p in $${allprogs}; do \
	case $$p in \
		=*) $(ECHO); $(ECHO) "$$p";; \
		*) \
			$(ECHO) -n "$$p:$$spaces" | $(SED) -e 's/^\(.\{0,20\}\).*$$/\1/'; \
			loc=`$(WHICH) $$p`; \
			if [ x"$$?" = x"0" ]; then \
				$(ECHO) "$(C_SUCCESS)Found:$(C_RESET) $$loc"; \
			else \
				$(ECHO) "$(C_FAILURE)Not Found$(C_RESET)"; \
			fi; \
			;; \
	esac; \
	done

.PHONY: _check_gpi_files
_check_gpi_files:
	$(QUIET)$(ECHO) "== Checking all .gpi files for common errors =="; \
	$(ECHO); \
	for f in $(files.gpi); do \
	result=`$(EGREP) '^([^#]*set terminal |set output )' $$f`; \
	$(ECHO) -n "$$f: "; \
	if [ x"$$result" = x"" ]; then \
		$(ECHO) "$(C_SUCCESS)Okay$(C_RESET)"; \
	else \
		$(ECHO) "$(C_FAILURE)Warning: Problematic commands:$(C_RESET)";\
		$(ECHO) "$(C_ERROR)$$result$(C_RESET)"; \
	fi; \
	done; \
	$(ECHO)

.PHONY: _all_stems
_all_stems:
	$(QUIET)$(ECHO) "== All Stems =="
	$(QUIET)$(call echo-list,$(sort $(default_stems_ss)))

.PHONY: _includes
_includes:
	$(QUIET)$(ECHO) "== Include Stems =="
	$(QUIET)$(ECHO) "=== Sources ==="
	$(QUIET)$(call echo-list,$(sort $(source_includes)))
	$(QUIET)$(ECHO) "=== Graphics ==="
	$(QUIET)$(call echo-list,$(sort $(graphic_includes)))

.PHONY: _all_sources
_all_sources:
	$(QUIET)$(ECHO) "== All Sources =="
	$(QUIET)$(call echo-list,$(sort $(all_files.tex)))

.PHONY: _dependency_graph
_dependency_graph:
	$(QUIET)$(ECHO) "/* LaTeX Dependency Graph */"
	$(QUIET)$(call output-dependency-graph)

.PHONY: _show_dependency_graph
_show_dependency_graph:
	$(QUIET)$(call output-dependency-graph,$(graph_stem).dot)
	$(QUIET)$(DOT) -Tps -o $(graph_stem).eps $(graph_stem).dot
	$(QUIET)$(VIEW_POSTSCRIPT) $(graph_stem).eps
	$(QUIET)$(call remove-temporary-files,$(graph_stem).*)

.PHONY: _sources
_sources:
	$(QUIET)$(ECHO) "== Sources =="
	$(QUIET)$(call echo-list,$(sort $(files.tex)))

.PHONY: _scripts
_scripts:
	$(QUIET)$(ECHO) "== Scripts =="
	$(QUIET)$(call echo-list,$(sort $(files_scripts)))

.PHONY: _graphic_outputs
_graphic_outputs:
	$(QUIET)$(ECHO) "== Graphic Outputs =="
	$(QUIET)$(call echo-list,$(sort $(all_graphics_targets)))

.PHONY: _env
_env:
ifdef .VARIABLES
	$(QUIET)$(ECHO) "== MAKE VARIABLES =="
	$(QUIET)$(call echo-list,$(foreach var,$(sort $(.VARIABLES)),'$(var)'))
endif
	$(QUIET)$(ECHO) "== ENVIRONMENT =="
	$(QUIET)$(ENV)

#
# CLEAN TARGETS
#
# clean-generated is somewhat unique - it relies on the .fls file being
# properly built so that it can determine which of the files was generated, and
# which was not.  Expect it to silently fail if the .fls file is missing.
#
# This is used to, e.g., clean up index files that are generated by the LaTeX.
.PHONY: clean-generated
clean-generated:
	$(QUIET)$(call clean-files,$(foreach e,$(addsuffix .fls,$(all_stems_source)),\
						$(shell $(call get-generated-names,$e))))

.PHONY: clean-deps
clean-deps:
	$(QUIET)$(call clean-files,$(all_d_targets) *.make *.make.temp *.cookie)

.PHONY: clean-tex
clean-tex: clean-deps
	$(QUIET)$(call clean-files,$(rm_tex))

.PHONY: clean-graphics
# TODO: This *always* deletes pstex files, even if they were not generated by
# anything....  In other words, if you create a pstex and pstex_t pair by hand
# an drop them in here without the generating fig file, they will be deleted
# and you won't get them back.  It's a hack put in here because I'm not sure we
# even want to keep pstex functionality, so my motivation is not terribly high
# for doing it right.
clean-graphics:
	$(QUIET)$(call clean-files,$(all_graphics_targets) *.gpi.d *.pstex *.pstex_t *.dot_t)

.PHONY: clean-backups
clean-backups:
	$(QUIET)$(call clean-files,$(backup_patterns) *.temp)

.PHONY: clean-auxiliary
clean-auxiliary:
	$(QUIET)$(call clean-files,$(graph_stem).*)

.PHONY: clean-nographics
clean-nographics: clean-tex clean-deps clean-backups clean-auxiliary ;

.PHONY: clean
clean: clean-generated clean-tex clean-graphics clean-deps clean-backups clean-auxiliary ;

#
# HELP TARGETS
#

.PHONY: help
help:
	$(help_text)

.PHONY: version
version:
	$(QUIET)\
	$(ECHO) "$(fileinfo) Version $(version)"; \
	$(ECHO) "by $(author)"; \

#
# HELP TEXT
#

define help_text
# $(fileinfo) Version $(version)
#
# by $(author)
#
# Generates a number of possible output files from a LaTeX document and its
# various dependencies.  Handles .bib files, \include and \input, and .eps
# graphics.  All dependencies are handled automatically by running LaTeX over
# the source.
#
# USAGE:
#
#    make [GRAY=1] [VERBOSE=1] [SHELL_DEBUG=1] <target(s)>
#
# STANDARD OPTIONS:
#    GRAY:
#        Setting this variable forces all recompiled graphics to be grayscale.
#        It is useful when creating a document for printing.  The default is
#        to allow colors.  Note that it only changes graphics that need to be
#        rebuilt!  It is usually a good idea to do a 'make clean' first.
#
#    VERBOSE:
#        This turns off all @ prefixes for commands invoked by make.  Thus,
#        you get to see all of the gory details of what is going on.
#
#    SHELL_DEBUG:
#        This enables the -x option for sh, meaning that everything it does is
#        echoed to stderr.  This is particularly useful for debugging
#        what is going on in $$(shell ...) invocations.  One of my favorite
#        debugging tricks is to do this:
#
#        make -d SHELL_DEBUG=1 VERBOSE=1 2>&1 | less
#
#    KEEP_TEMP:
#        When set, this allows .make and other temporary files to stick around
#        long enough to do some debugging.  This can be useful when trying to
#        figure out why gnuplot is not doing the right things, for example
#        (e.g., look for *head.make).
#
# STANDARD AUXILIARY FILES:
#
#      Variables.ini (formerly Makefile.ini, which still works)
#
#          This file can contain variable declarations that override various
#          aspects of the makefile.  For example, one might specify
#
#          neverclean := *.pdf *.ps
#          onlysources.tex := main.tex
#          LATEX_COLOR_WARNING := 'bold red uline'
#
#          And this would override the neverclean setting to ensure that pdf
#          and ps files always remain behind, set the makefile to treat all
#          .tex files that are not "main.tex" as includes (and therefore not
#          default targets).  It also changes the LaTeX warning output to be
#          red, bold, and underlined.
#
#          There are numerous variables in this file that can be overridden in
#          this way.  Search for '?=' to find them all.
#
#          The Variables.ini is imported before *anything else* is done, so go
#          wild with your ideas for changes to this makefile in there.  It
#          makes it easy to test them before submitting patches.
#
#          If you're adding rules or targets, however, see Targets.ini below.
#
#      Targets.ini
#
#          This is included much later in the makefile, after all variables and
#          targets are defined.  This is where you would put new make rules,
#          e.g.,
#
#          generated.tex: generating_script.weird_lang depA depB
#             ./generating_script.weird_lang > $$@
#
#          In this file, you have access to all of the variables that the
#          makefile creates, like $(onlysources.tex).  While accessing those can
#          be somewhat brittle (they are implementation details and may change),
#          it is a great way to test your ideas when submitting feature requests.
#
# STANDARD ENVIRONMENT VARIABLES:
#
#      LATEX_COLOR_WARNING        '$(LATEX_COLOR_WARNING)'
#      LATEX_COLOR_ERROR          '$(LATEX_COLOR_ERROR)'
#      LATEX_COLOR_UNDERFULL      '$(LATEX_COLOR_UNDERFULL)'
#      LATEX_COLOR_OVERFULL       '$(LATEX_COLOR_OVERFULL)'
#      LATEX_COLOR_PAGES          '$(LATEX_COLOR_PAGES)'
#      LATEX_COLOR_BUILD          '$(LATEX_COLOR_BUILD)'
#      LATEX_COLOR_GRAPHIC        '$(LATEX_COLOR_GRAPHIC)'
#      LATEX_COLOR_DEP            '$(LATEX_COLOR_DEP)'
#      LATEX_COLOR_SUCCESS        '$(LATEX_COLOR_SUCCESS)'
#      LATEX_COLOR_FAILURE        '$(LATEX_COLOR_FAILURE)'
#
#   These may be redefined in your environment to be any of the following:
#
#      black
#      red
#      green
#      yellow
#      blue
#      magenta
#      cyan
#      white
#
#   Bold or underline may be used, as well, either alone or in combination
#   with colors:
#
#      bold
#      uline
#
#   Order is not important.  You may want, for example, to specify:
#
#   export LATEX_COLOR_SUCCESS='bold blue uline'
#
#   in your .bashrc file.  I don't know why, but you may want to.
#
# STANDARD TARGETS:
#
#    all:
#        Make all possible documents in this directory.  The documents are
#        determined by scanning for .tex and .tex.sh (described in more detail
#        later) and omitting any file that ends in ._include_.tex or
#        ._nobuild_.tex.  The output is a set of .pdf files.
#
#        If you wish to omit files without naming them with the special
#        underscore names, set the following near the top of the Makefile,
#        or (this is recommended) within a Makefile.ini in the same directory:
#
#         includes.tex := file1.tex file2.tex
#
#        This will cause the files listed to be considered as include files.
#
#        If you have only few source files, you can set
#
#         onlysources.tex := main.tex
#
#        This will cause only the source files listed to be considered in
#        dependency detection.  All other .tex files will be considered as
#        include files.  Note that these options work for *any* source type,
#        so you could do something similar with includes.gpi, for example.
#        Note that this works for *any valid source* target.  All of the
#        onlysources.* variables are commented out in the shipping version of
#        this file, so it does the right thing when they simply don't exist.
#        The comments are purely documentation.  If you know, for example, that
#        file.mycoolformat is supported by this Makefile, but don't see the
#        "onlysources.mycoolformat" declared in the comments, that doesn't mean
#        you can't use it.  Go ahead and set "onlysources.mycoolformat" and it
#        should do the right thing.
#
#    show:
#        Builds and displays all documents in this directory.  It uses the
#        environment-overridable value of VIEW_PDF (currently $(VIEW_PDF)) to
#        do its work.
#
#    all-graphics:
#        Make all of the graphics in this directory.
#
#    all-pstex (only for BUILD_STRATEGY=latex):
#        Build all fig files into pstex and pstex_t files.  Gray DOES NOT WORK.
#
#    all-gray-pstex (only for BUILD_STRATEGY=latex):
#          Build all fig files into grayscale pstex and pstex_t files.
#
#    all-dot2tex:
#          Build all dot files into tex files.
#
#    show-graphics:
#        Builds and displays all graphics in this directory.  Uses the
#        environment-overridable value of VIEW_GRAPHICS (currently
#        $(VIEW_GRAPHICS)) to do its work.
#
#    clean:
#        Remove ALL generated files, leaving only source intact.
#        This will *always* skip files mentioned in the "neverclean" variable,
#        either in this file or specified in Makefile.ini:
#
#         neverclean := *.pdf *.ps
#
#       The neverclean variable works on all "clean" targets below, as well.
#
#    clean-graphics:
#        Remove all generated graphics files.
#
#    clean-backups:
#        Remove all backup files: $(backup_patterns)
#        (XFig and other editors have a nasty habit of leaving them around)
#        Also removes Makefile-generated .temp files
#
#    clean-tex:
#        Remove all files generated from LaTeX invocations except dependency
#        information.  Leaves graphics alone.
#
#    clean-deps:
#        Removes all auto-generated dependency information.
#
#    clean-auxiliary:
#        Removes extra files created by various targets (like the dependency
#        graph output).
#
#    clean-nographics:
#        Cleans everything *except* the graphics files.
#
#    help:
#        This help text.
#
#    version:
#        Version information about this LaTeX makefile.
#
# DEBUG TARGETS:
#
#    _all_programs:
#        A list of the programs used by this makefile.
#
#    _check_programs:
#        Checks your system for the needed software and reports what it finds.
#
#    _check_gpi_files:
#        Checks the .gpi files in the current directory for common errors, such
#        as specification of the terminal or output file inside of the gpi file
#        itself.
#
#    _dependency_graph:
#        Outputs a .dot file to stdout that represents a graph of LaTeX
#        dependencies.  To see it, use the _show_dependency_graph target or
#        direct the output to a file, run dot on it, and view the output, e.g.:
#
#        make _dependency_graph > graph.dot
#        dot -T ps -o graph.eps graph.dot
#        gv graph.eps
#
#    _show_dependency_graph:
#        Makes viewing the graph simple: extracts, builds and displays the
#        dependency graph given in the _dependency_graph target using the value
#        of the environment-overridable VIEW_POSTSCRIPT variable (currently set
#        to $(VIEW_POSTSCRIPT)).  The postscript viewer is used because it
#        makes it easier to zoom in on the graph, a critical ability for
#        something so dense and mysterious.
#
#    _all_sources:
#        List all .tex files in this directory.
#
#    _sources:
#        Print out a list of all compilable sources in this directory.  This is
#        useful for determining what make thinks it will be using as the
#        primary source for 'make all'.
#
#    _scripts:
#        Print out a list of scripts that make knows can be used to generate
#        .tex files (described later).
#
#    _all_stems:
#        Print a list of stems.  These represent bare targets that can be
#        executed.  Listing <stem> as a bare target will produce <stem>.pdf.
#
#    _includes:
#        A list of .d files that would be included in this run if _includes
#        weren't specified.  This target may be used alone or in conjunction
#        with other targets.
#
#    _graphic_outputs:
#        A list of all generated .eps files
#
#    _env:
#        A list of environment variables and their values.  If supported by
#        your version of make, also a list of variables known to make.
#
# FILE TARGETS:
#
#    %, %.pdf:
#        Build a PDF file from the corresponding %.tex file.
#
#        If BUILD_STRATEGY=pdflatex, then this builds the pdf directly.
#        Otherwise, it uses this old-school but effective approach:
#
#            latex -> dvips -> ps2pdf
#
#        The BUILD_STRATEGY can be overridden in Makefile.ini in the same
#        directory.  The default is pdflatex.
#
#        Reasons for using latex -> dvips include the "psfrag" package, and the
#        generation of postscript instead of PDF.  Arguments for using pdflatex
#        include "new and shiny" and "better supported."  I can't argue with
#        either of those, and supporting them both didn't turn out to be that
#        difficult, so there you have it.  Choices.
#
#    %._show:
#        A phony target that builds the pdf file and then displays it using the
#        environment-overridable value of VIEW_PDF ($(VIEW_PDF)).
#
#    %._graphics:
#        A phony target that generates all graphics on which %.pdf (or %.dvi)
#        depends.
#
#    %.ps (only for BUILD_STRATEGY=latex):
#        Build a Postscript file from the corresponding %.tex file.
#        This is done using dvips.  Paper size is automatically
#        extracted from the declaration
#
#        \documentclass[<something>paper]
#
#        or it is the system default.
#
#        If using beamer (an excellent presentation class), the paper
#        size is ignored.  More on this later.
#
#    %.dvi (only for BUILD_STRATEGY=latex):
#        Build the DVI file from the corresponding %.tex file.
#
#    %.ind:
#        Build the index for this %.tex file.
#
#    %.gls:
#        Build the nomenclature glossary for this %.tex file.
#
#    %.nls:
#        Build the (newer) nomenclature file for this %.tex file.
#
#    %.eps:
#        Build an eps file from one of the following file types:
#
#       .dot    : graphviz
#       .gpi    : gnuplot
#       .fig    : xfig
#       .xvg    : xmgrace
#       .svg    : scalable vector graphics (goes through inkscape)
#       .png    : png (goes through NetPBM)
#       .jpg      : jpeg (goes through ImageMagick)
#       .eps.gz : gzipped eps
#
#       The behavior of this makefile with each type is described in
#       its own section below.
#
#    %.pstex{,_t} (only for BUILD_STRATEGY=latex):
#       Build a .pstex_t file from a .fig file.
#
# FEATURES:
#
#    Optional Binary Directory:
#        If you create the _out_ directory in the same place as the makefile,
#        it will automatically be used as a dumping ground for .pdf (or .dvi,
#        .ps, and .pdf) output files.
#
#        Alternatively, you can set the BINARY_TARGET_DIR variable, either as a
#        make argument or in Makefile.ini, to point to your directory of
#        choice.  Note that no pathname wildcard expansion is done in the
#        makefile, so make sure that the path is complete before going in
#        there.  E.g., if you want to specify something in your home directory,
#        use $$HOME/ instead of ~/ so that the shell expands it before it gets
#        to the makefile.
#
#    External Program Dependencies:
#        Every external program used by the makefile is represented by an
#        ALLCAPS variable at the top of this file.  This should allow you to
#        make judgments about whether your system supports the use of this
#        makefile.  The list is available in the ALL_PROGRAMS variable and,
#        provided that you are using GNU make 3.80 or later (or you haven't
#        renamed this file to something weird like "mylatexmakefile" and like
#        invoking it with make -f) can be viewed using
#
#        make _all_programs
#
#        Additionally, the availability of these programs can be checked
#        automatically for you by running
#
#        make _check_programs
#
#        The programs are categorized according to how important they are and
#        what function they perform to help you decide which ones you really
#        need.
#
#    Colorized Output:
#        The output of commands is colorized to highlight things that are often
#        important to developers.  This includes {underfull,overfull}
#        {h,v}boxes, general LaTeX Errors, each stage of document building, and
#        the number of pages in the final document.  The colors are obtained
#        using 'tput', so colorization should work pretty well on any terminal.
#
#        The colors can be customized very simply by setting any of the
#        LATEX_COLOR_<CONTEXT> variables in your environment (see above).
#
#    Predecessors to TeX Files:
#        Given a target <target>, if no <target>.tex file exists but a
#        corresponding script or predecessor file exists, then appropriate
#        action will be taken to generate the tex file.
#
#        Currently supported script or predecessor languages are:
#
#        sh:     %.tex.sh
#        perl:   %.tex.pl
#        python: %.tex.py
#
#           Calls the script using the appropriate interpreter, assuming that
#           its output is a .tex file.
#
#           The script is called thus:
#
#              <interpreter> <script file name> <target tex file>
#
#           and therefore sees exactly one parameter: the name of the .tex
#           file that it is to create.
#
#           Why does this feature exist?  I ran into this while working on
#           my paper dissertation.  I wrote a huge bash script that used a
#           lot of sed to bring together existing papers in LaTeX.  It
#           would have been nice had I had something like this to make my
#           life easier, since as it stands I have to run the script and
#           then build the document with make.  This feature provides hooks
#           for complicated stuff that you may want to do, but that I have
#           not considered.  It should work fine with included dependencies,
#           too.
#
#           Scripts are run every time make is invoked.  Some trickery is
#           employed to make sure that multiple restarts of make don't cause
#           them to be run again.
#
#        reST: %.rst
#
#           Runs the reST to LaTeX converter to generate a .tex file
#           If it finds a file names _rststyle_._include_.tex, uses it as
#           the "stylesheet" option to rst2latex.
#
#           Note that this does not track sub-dependencies in rst files.  It
#           assumes that the top-level rst file will change if you want a
#           rebuild.
#
#    Dependencies:
#
#        In general, dependencies are extracted directly from LaTeX output on
#        your document.  This includes
#
#        *    Bibliography information
#        *    \include or \input files (honoring \includeonly, too)
#        *    Graphics files inserted by the graphicx package
#
#        Where possible, all of these are built correctly and automatically.
#        In the case of graphics files, these are generated from the following
#        file types:
#
#        GraphViz:      .dot
#        GNUPlot:       .gpi
#        XFig:          .fig
#        XMgrace:       .xvg
#        SVG:           .svg
#        PNG:           .png
#        JPEG:          .jpg
#        GZipped EPS:   .eps.gz
#
#        If the file exists as a .eps already, it is merely used (and will not
#        be deleted by 'clean'!).
#
#        LaTeX and BibTeX are invoked correctly and the "Rerun to get
#        cross-references right" warning is heeded a reasonable number of
#        times.  In my experience this is enough for even the most troublesome
#        documents, but it can be easily changed (if LaTeX has to be run after
#        BibTeX more than three times, it is likely that something is moving
#        back and forth between pages, and no amount of LaTeXing will fix
#        that).
#
#        \includeonly is honored by this system, so files that are not
#        specified there will not trigger a rebuild when changed.
#
#    Beamer:
#        A special TeX source comment is recognized by this makefile (only when
#        BUILD_STRATEGY=latex, since this invokes psnup):
#
#        %%[[:space:]]*BEAMER[[:space:]]*LARGE
#
#        The presence of this comment forces the output of dvips through psnup
#        to enlarge beamer slides to take up an entire letter-sized page.  This
#        is particularly useful when printing transparencies or paper versions
#        of the slides.  For some reason landscape orientation doesn't appear
#        to work, though.
#
#        If you want to put multiple slides on a page, use this option and then
#        print using mpage, a2ps, or psnup to consolidate slides.  My personal
#        favorite is a2ps, but your mileage may vary.
#
#        When beamer is the document class, dvips does NOT receive a paper size
#        command line attribute, since beamer does special things with sizes.
#
#    GNUPlot Graphics:
#        When creating a .gpi file, DO NOT INCLUDE the "set terminal" or "set
#        output" commands!  The makefile will include terminal information for
#        you.  Besides being unnecessary and potentially harmful, including the
#        terminal definition in the .gpi file makes it harder for you, the one
#        writing the document, to preview your graphics, e.g., with
#
#           gnuplot -persist myfile.gpi
#
#        so don't do specify a terminal or an output file in your .gpi files.
#
#        When building a gpi file into an eps file, there are several features
#        available to the document designer:
#
#        Global Header:
#            The makefile searches for the files in the variable GNUPLOT_GLOBAL
#            in order:
#
#            ($(GNUPLOT_GLOBAL))
#
#            Only the first found is used.  All .gpi files in the directory are
#            treated as though the contents of GNUPLOT_GLOBAL were directly
#            included at the top of the file.
#
#            NOTE: This includes special comments! (see below)
#
#        Font Size:
#            A special comment in a .gpi file (or a globally included file) of
#            the form
#
#            ## FONTSIZE=<number>
#
#            will change the font size of the GPI output.  If font size is
#            specified in both the global file and the GPI file, the
#            specification in the individual GPI file is used.
#
#        Grayscale Output:
#            GNUplot files also support a special comment to force them to be
#            output in grayscale *no matter what*:
#
#            ## GRAY
#
#            This is not generally advisable, since you can always create a
#            grayscale document using the forms mentioned above.  But, if your
#            plot simply must be grayscale even in a document that allows
#            colors, this is how you do it.
#
#    XFig Graphics:
#            No special handling is done with XFig, except when a global
#            grayscale method is used, e.g.
#
#                make GRAY=1 document
#
#            In these cases the .eps files is created using the -N switch to
#            fig2dev to turn off color output.  (Only works with eps, not pstex
#            output)
#
#    GraphVis Graphics:
#            Color settings are simply ignored here.  The 'dot' program is used
#            to transform a .dot file into a .eps file.
#
#            If you want, you can use the dot2tex program to convert dot files
#            to tex graphics.  The default is to just call dot2tex with no
#            arguments, but you can change the DOT2TEX definition to include
#            options as needed (in your Makefile.ini).
#
#            Note that, as with pstex, the makefile cannot use latex's own
#            output to discover all missing dot_t (output) files, since anytime
#            TeX includes TeX, it has to bail when it can't find the include
#            file.  It can therefore only stop on the first missing file it
#            discovers, and we can't get a large list of them out easily.
#
#            So, the makefile errors out if it's missing an included dot_t
#            file, then prompts the user to run this command manually:
#
#                make all-dot2tex
#
#    GZipped EPS Graphics:
#
#        A .eps.gz file is sometimes a nice thing to have.  EPS files can get
#        very large, especially when created from bitmaps (don't do this if you
#        don't have to).  This makefile will unzip them (not in place) to
#        create the appropriate EPS file.
#
#
endef

#
# DEPENDENCY CHART:
#
# digraph "g" {
#     rankdir=TB
#     size="9,9"
#     edge [fontsize=12 weight=10]
#     node [shape=box fontsize=14 style=rounded]
#
#     eps [
#         shape=Mrecord
#         label="{{<gpi> GNUplot|<epsgz> GZip|<dot> Dot|<fig> XFig}|<eps> eps}"
#         ]
#     pstex [label="%.pstex"]
#     pstex_t [label="%.pstex_t"]
#     tex_outputs [shape=point]
#     extra_tex_files [shape=point]
#     gpi_data [label="<data>"]
#     gpi_includes [label="_include_.gpi"]
#     aux [label="%.aux"]
#     fls [label="%.fls"]
#     idx [label="%.idx"]
#     glo [label="%.glo"]
#     ind [label="%.ind"]
#     log [label="%.log"]
#     tex_sh [label="%.tex.sh"]
#     rst [label="%.rst"]
#     tex [
#         shape=record
#         label="<tex> %.tex|<include> _include_.tex"
#         ]
#     include_aux [label="_include_.aux"]
#     file_bib [label=".bib"]
#     bbl [label="%.bbl"]
#     dvi [label="%.dvi"]
#     ps [label="%.ps"]
#     pdf [label="%.pdf"]
#     fig [label=".fig"]
#     dot [label=".dot"]
#     gpi [label=".gpi"]
#     eps_gz [label=".eps.gz"]
#
#     gpi_files [shape=point]
#
#     rst -> tex:tex [label="reST"]
#     tex_sh -> tex:tex [label="sh"]
#     tex_pl -> tex:tex [label="perl"]
#     tex_py -> tex:tex [label="python"]
#     tex -> tex_outputs [label="latex"]
#     tex_outputs -> dvi
#     tex_outputs -> aux
#     tex_outputs -> log
#     tex_outputs -> fls
#     tex_outputs -> idx
#     tex_outputs -> include_aux
#     aux -> bbl [label="bibtex"]
#     file_bib -> bbl [label="bibtex"]
#     idx -> ind [label="makeindex"]
#     glo -> gls [label="makeindex"]
#     nlo -> nls [label="makeindex"]
#     gls -> extra_tex_files
#     nls -> extra_tex_files
#     ind -> extra_tex_files
#     bbl -> extra_tex_files
#     eps -> extra_tex_files
#     extra_tex_files -> dvi [label="latex"]
#     gpi_files -> eps:gpi [label="gnuplot"]
#     gpi -> gpi_files
#     gpi_data -> gpi_files
#     gpi_includes -> gpi_files
#     eps_gz -> eps:epsgz [label="gunzip"]
#     fig -> eps:fig [label="fig2dev"]
#     fig -> pstex [label="fig2dev"]
#     fig -> pstex_t [label="fig2dev"]
#     pstex -> pstex_t [label="fig2dev"]
#     dot -> eps:dot [label="dot"]
#     dvi -> ps [label="dvips"]
#     include_aux -> bbl [label="bibtex"]
#     ps -> pdf [label="ps2pdf"]
#
#     edge [ color=blue label="" style=dotted weight=1 fontcolor=blue]
#     fls -> tex:include [label="INPUT: *.tex"]
#     fls -> file_bib [label="INPUT: *.aux"]
#     aux -> file_bib [label="\\bibdata{...}"]
#     include_aux -> file_bib [label="\\bibdata{...}"]
#     log -> gpi [label="Graphic file"]
#     log -> fig [label="Graphic file"]
#     log -> eps_gz [label="Graphic file"]
#     log -> dot [label="Graphic file"]
#     log -> idx [label="No file *.ind"]
#     log -> glo [label="No file *.gls"]
#     log -> nlo [label="No file *.nls"]
#     gpi -> gpi_data [label="plot '...'"]
#     gpi -> gpi_includes [label="load '...'"]
#     tex:tex -> ps [label="paper"]
#     tex:tex -> pdf [label="embedding"]
# }
#

#
# DEPENDENCY CHART SCRIPT
#
# $(call output_dependency_graph,[<output file>])
define output-dependency-graph
	if [ -f '$(this_file)' ]; then \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*DEPENDENCY CHART:/,/^$$/!d' \
		-e '/DEPENDENCY CHART/d' \
		-e '/^$$/d' \
		-e 's/^[[:space:]]*#//' \
		$(this_file) $(if $1,> '$1',); \
	else \
		$(ECHO) "Cannot determine the name of this makefile."; \
	fi
endef
#
.PHONY: Targets.ini $(HOME)/.latex-makefile/Targets.ini
-include Targets.ini
-include $(HOME)/.latex-makefile/Targets.ini
#
# vim: noet sts=0 sw=8 ts=8



==> dft-tikz.tex <==

\makeatletter

\pgfdeclareshape{spare}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northeast}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -1\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spare/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spare/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spare node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,fill=white!100!black,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{spareM}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northwest}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@xa by -1\pgf@x
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spareM/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spareM/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spareM node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{fdep}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{EA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{ED}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{T}{ % trigger anchor
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@fdep@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % trinagle input
    \pgf@anchor@fdep@T
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.3333\pgf@x
    \advance\pgf@xb by -.5\pgf@x
    \advance\pgf@yb by .\pgf@x
    \advance\pgf@yc by .3333\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{fdep/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@fdep@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@ED
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{fdep/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every fdep node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\newif\ifpgfshapebaselesstrianglehasinline
\newif\ifpgfshapebaselesstriangleclose
\pgfkeys{/pgf/.cd,
  baseless triangle apex angle/.style={/pgf/isosceles triangle apex angle=#1},
  baseless triangle inline/.is if=pgfshapebaselesstrianglehasinline,
  baseless triangle has base/.is if=pgfshapebaselesstriangleclose
}

\pgfdeclareshape{baseless triangle}{
  % Copy some stuff from the isosecles triangle
  \inheritsavedanchors[from={isosceles triangle}]
  \inheritanchor[from={isosceles triangle}]{center}
  \inheritanchor[from={isosceles triangle}]{north}
  \inheritanchor[from={isosceles triangle}]{south}
  \inheritanchor[from={isosceles triangle}]{east}
  \inheritanchor[from={isosceles triangle}]{west}
  \inheritanchorborder[from={isosceles triangle}]
  \backgroundpath{%
    % The isoceles triangle defines lots of parameters
    % in the \trianglepoints macro.
        \trianglepoints%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            % This bit is a bit of a kludge to ensure the inline
            % is at the top of the figure.
            \pgftransformyscale{cos(\rotate)}%
            \pgfpathmoveto{\lowerleft}%
            \pgfpathlineto{\apex}%
            \pgfpathlineto{\lowerleft\pgf@y=-\pgf@y}%
            % Close the base?
            \ifpgfshapebaselesstriangleclose%
              \pgfpathclose%
            \fi%
            % Draw the inline?
            \ifpgfshapebaselesstrianglehasinline
              \pgfpointdiff{\lowerleft}%
                 {\pgfpointlineattime{0.125}{\lowerleft}{\lowerleft\pgf@y=-\pgf@y}}%
                \pgfgetlastxy{\x}{\y}%
                \pgfmathveclen{\x}{\y}%
                \let\inlineshift=\pgfmathresult%
            % Calculate where the inline hits the sloped line of the triangle.
            \pgfmathparse{\inlineshift/2/sin(\pgfkeysvalueof{/pgf/isosceles triangle apex angle}/2)}%
            \let\inlineendshift=\pgfmathresult
            \pgfpathmoveto{\pgfpointadd{\pgfpoint{0pt}{-\inlineshift}}{\lowerleft}}%
            \pgfpathlineto{\pgfpointlineatdistance{\inlineendshift}{\apex}{\lowerleft}\pgf@y=-\pgf@y}%
        \fi%
    }
    }
}





\makeatother

\tikzstyle{every picture}=[>=stealth]
\tikzstyle{fdarrow}=[>=triangle 60,double,double equal sign distance,-implies,dashed]
\tikzstyle{and1}=[and gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{and2}=[and gate US,draw,  shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{and3}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and4}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{and5}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{and6}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.7]
\tikzstyle{or1}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{or2}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{or3}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or4}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{or5}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{or6}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{be}=[circle,draw,fill=white!100,anchor=north, inner sep=5pt, minimum width=0.7cm]
\tikzstyle{cnst}=[diamond,draw,fill=white!100,anchor=north, minimum width=0.5cm,font=\scriptsize, scale=0.8]
\tikzstyle{seq}=[rectangle,draw,fill=white!100, minimum width=0.7cm,font=\LARGE, inner sep=3pt]
\tikzstyle{labelbox} = [rectangle, draw, inner sep=2pt, anchor=south, minimum width=0.6cm, minimum height=0.4cm, scale=0.8]
\tikzstyle{transfer} = [isosceles triangle, draw, shape border rotate=90, inner sep=2pt, minimum width=0.9cm, minimum height=0.7cm, isosceles triangle stretches=true]

\tikzstyle{triangle}=[isosceles triangle,draw,shape border rotate=90,isosceles triangle stretches=true, minimum height=0.6cm,minimum width=0.6cm]
\tikzstyle{btriangle}=[baseless triangle,draw,rotate=90, minimum height=0.6cm]

\tikzstyle{failed}=[draw=red!60!black!100, fill=red!05]

